Bayesian inference methodology for Primordial Power Spectrum reconstructions from Large Scale Structure

We use Bayesian inference and nested sampling to develop a non-parametric method to reconstruct the primordial power spectrum $P_{\mathcal{R}}(k)$ from Large Scale Structure (LSS) data. The performance of the method is studied by applying it to simulations of the clustering of two different object catalogues, low-$z$ (ELGs) and high-$z$ (QSOs), and considering two different photometric errors. These object clusterings are derived from different templates of the primordial power spectrum motivated by models of inflation: the Standard Model power law characterized by the two parameters $A_s$ and $n_s$; a local feature template; and a global oscillatory template. Our reconstruction method involves sampling $N$ knots in the log $\{k,P_{\mathcal{R}}(k)\}$ plane. We use two statistical tests to examine the reconstructions for signs of primordial features: a global test comparing the evidences and a novel local test quantifying the power of the hypothesis test between the power law model and the marginalized probability over $N$ model. The method shows good performance in all scenarios considered. In particular, the tests show no feature detection for the SM. The method is able to detect power spectrum deviations at a level of $\approx 2\%$ for all considered features, combining either the low-$z$ or the high-$z$ redshift bins. Other scenarios with different redshift bins, photometric errors, feature amplitudes and detection levels are also discussed. In addition, we include a first application to real data from the Sloan Digital Sky Survey Luminous Red Galaxy Data Release 4 (SDSS LRG 04), finding no preference for deviations from the primordial power law. The method is flexible, model independent, and suitable for its application to existing and future LSS catalogues.

==> bibsecurity.tex <==
@ARTICLE{WillPaper,
       author = {{Handley}, Will J. and {Lasenby}, Anthony N. and {Peiris}, Hiranya V. and
         {Hobson}, Michael P.},
        title = "{Bayesian inflationary reconstructions from  2018 data}",
      journal = {\prd},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics, General Relativity and Quantum Cosmology},
         year = 2019,
        month = nov,
       volume = {100},
       number = {10},
          eid = {103511},
        pages = {103511},
          doi = {10.1103/PhysRevD.100.103511},
archivePrefix = {arXiv},
       eprint = {1908.00906},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019PhRvD.100j3511H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{SDSSLRG04,
       author = {{Tegmark}, Max and {Eisenstein}, Daniel J. and {Strauss}, Michael A. and
         {Weinberg}, David H. and {Blanton}, Michael R. and
         {Frieman}, Joshua A. and {Fukugita}, Masataka and {Gunn}, James E. and
         {Hamilton}, Andrew J.~S. and {Knapp}, Gillian R. and
         {Nichol}, Robert C. and {Ostriker}, Jeremiah P. and
         {Padmanabhan}, Nikhil and {Percival}, Will J. and {Schlegel}, David J. and
         {Schneider}, Donald P. and {Scoccimarro}, Roman and
         {Seljak}, Uro{\v{s}} and {Seo}, Hee-Jong and {Swanson}, Molly and
         {Szalay}, Alexander S. and {Vogeley}, Michael S. and {Yoo}, Jaiyul and
         {Zehavi}, Idit and {Abazajian}, Kevork and {Anderson}, Scott F. and
         {Annis}, James and {Bahcall}, Neta A. and {Bassett}, Bruce and
         {Berlind}, Andreas and {Brinkmann}, Jon and {Budavari}, Tam{\'a}s and
         {Castander}, Francisco and {Connolly}, Andrew and {Csabai}, Istvan and
         {Doi}, Mamoru and {Finkbeiner}, Douglas P. and {Gillespie}, Bruce and
         {Glazebrook}, Karl and {Hennessy}, Gregory S. and {Hogg}, David W. and
         {Ivezi{\'c}}, {\v{Z}}eljko and {Jain}, Bhuvnesh and {Johnston}, David and
         {Kent}, Stephen and {Lamb}, Donald Q. and {Lee}, Brian C. and
         {Lin}, Huan and {Loveday}, Jon and {Lupton}, Robert H. and
         {Munn}, Jeffrey A. and {Pan}, Kaike and {Park}, Changbom and
         {Peoples}, John and {Pier}, Jeffrey R. and {Pope}, Adrian and
         {Richmond}, Michael and {Rockosi}, Constance and {Scranton}, Ryan and
         {Sheth}, Ravi K. and {Stebbins}, Albert and {Stoughton}, Christopher and
         {Szapudi}, Istv{\'a}n and {Tucker}, Douglas L. and {vand
        en Berk}, Daniel E. and {Yanny}, Brian and {York}, Donald G.},
        title = "{Cosmological constraints from the SDSS luminous red galaxies}",
      journal = {\prd},
     keywords = {98.80.Es, Observational cosmology, Astrophysics, High Energy Physics - Phenomenology, High Energy Physics - Theory},
         year = 2006,
        month = dec,
       volume = {74},
       number = {12},
          eid = {123507},
        pages = {123507},
          doi = {10.1103/PhysRevD.74.123507},
archivePrefix = {arXiv},
       eprint = {astro-ph/0608632},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006PhRvD..74l3507T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Ref89SDSS,
       author = {{Eisenstein}, Daniel J. and {Hu}, Wayne},
        title = "{Power Spectra for Cold Dark Matter and Its Variants}",
      journal = {\apj},
     keywords = {COSMOLOGY: THEORY, COSMOLOGY: DARK MATTER, COSMOLOGY: LARGE-SCALE STRUCTURE OF UNIVERSE, Cosmology: Theory, Cosmology: Dark Matter, Cosmology: Large-Scale Structure of Universe, Astrophysics},
         year = 1999,
        month = jan,
       volume = {511},
       number = {1},
        pages = {5-15},
          doi = {10.1086/306640},
archivePrefix = {arXiv},
       eprint = {astro-ph/9710252},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ApJ...511....5E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ref88SDSS,
       author = {{Eisenstein}, Daniel J. and {Seo}, Hee-Jong and {White}, Martin},
        title = "{On the Robustness of the Acoustic Scale in the Low-Redshift Clustering of Matter}",
      journal = {\apj},
     keywords = {Cosmology: Cosmic Microwave Background, Cosmology: Cosmological Parameters, Cosmology: Distance Scale, Cosmology: Large-Scale Structure of Universe, Astrophysics},
         year = 2007,
        month = aug,
       volume = {664},
       number = {2},
        pages = {660-674},
          doi = {10.1086/518755},
archivePrefix = {arXiv},
       eprint = {astro-ph/0604361},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...664..660E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{SwitchingLabelProblem,
       author = {{Buscicchio}, Riccardo and {Roebber}, Elinore and {Goldstein}, Janna M. and
         {Moore}, Christopher J.},
        title = "{Label switching problem in Bayesian analysis for gravitational wave astronomy}",
      journal = {\prd},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2019,
        month = oct,
       volume = {100},
       number = {8},
          eid = {084041},
        pages = {084041},
          doi = {10.1103/PhysRevD.100.084041},
archivePrefix = {arXiv},
       eprint = {1907.11631},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019PhRvD.100h4041B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{PlanckInflation15,
       author = {{Planck Collaboration} and {Ade}, P.~A.~R. and {Aghanim}, N. and {Arnaud}, M. and {Arroja}, F. and {Ashdown}, M. and {Aumont}, J. and {Baccigalupi}, C. and {Ballardini}, M. and {Banday}, A.~J. and {Barreiro}, R.~B. and {Bartolo}, N. and {Battaner}, E. and {Benabed}, K. and {Beno{\^\i}t}, A. and {Benoit-L{\'e}vy}, A. and {Bernard}, J. -P. and {Bersanelli}, M. and {Bielewicz}, P. and {Bock}, J.~J. and {Bonaldi}, A. and {Bonavera}, L. and {Bond}, J.~R. and {Borrill}, J. and {Bouchet}, F.~R. and {Boulanger}, F. and {Bucher}, M. and {Burigana}, C. and {Butler}, R.~C. and {Calabrese}, E. and {Cardoso}, J. -F. and {Catalano}, A. and {Challinor}, A. and {Chamballu}, A. and {Chary}, R. -R. and {Chiang}, H.~C. and {Christensen}, P.~R. and {Church}, S. and {Clements}, D.~L. and {Colombi}, S. and {Colombo}, L.~P.~L. and {Combet}, C. and {Contreras}, D. and {Couchot}, F. and {Coulais}, A. and {Crill}, B.~P. and {Curto}, A. and {Cuttaia}, F. and {Danese}, L. and {Davies}, R.~D. and {Davis}, R.~J. and {de Bernardis}, P. and {de Rosa}, A. and {de Zotti}, G. and {Delabrouille}, J. and {D{\'e}sert}, F. -X. and {Diego}, J.~M. and {Dole}, H. and {Donzelli}, S. and {Dor{\'e}}, O. and {Douspis}, M. and {Ducout}, A. and {Dupac}, X. and {Efstathiou}, G. and {Elsner}, F. and {En{\ss}lin}, T.~A. and {Eriksen}, H.~K. and {Fergusson}, J. and {Finelli}, F. and {Forni}, O. and {Frailis}, M. and {Fraisse}, A.~A. and {Franceschi}, E. and {Frejsel}, A. and {Frolov}, A. and {Galeotta}, S. and {Galli}, S. and {Ganga}, K. and {Gauthier}, C. and {Giard}, M. and {Giraud-H{\'e}raud}, Y. and {Gjerl{\o}w}, E. and {Gonz{\'a}lez-Nuevo}, J. and {G{\'o}rski}, K.~M. and {Gratton}, S. and {Gregorio}, A. and {Gruppuso}, A. and {Gudmundsson}, J.~E. and {Hamann}, J. and {Handley}, W. and {Hansen}, F.~K. and {Hanson}, D. and {Harrison}, D.~L. and {Henrot-Versill{\'e}}, S. and {Hern{\'a}ndez-Monteagudo}, C. and {Herranz}, D. and {Hildebrandt}, S.~R. and {Hivon}, E. and {Hobson}, M. and {Holmes}, W.~A. and {Hornstrup}, A. and {Hovest}, W. and {Huang}, Z. and {Huffenberger}, K.~M. and {Hurier}, G. and {Jaffe}, A.~H. and {Jaffe}, T.~R. and {Jones}, W.~C. and {Juvela}, M. and {Keih{\"a}nen}, E. and {Keskitalo}, R. and {Kim}, J. and {Kisner}, T.~S. and {Kneissl}, R. and {Knoche}, J. and {Kunz}, M. and {Kurki-Suonio}, H. and {Lagache}, G. and {L{\"a}hteenm{\"a}ki}, A. and {Lamarre}, J. -M. and {Lasenby}, A. and {Lattanzi}, M. and {Lawrence}, C.~R. and {Leonardi}, R. and {Lesgourgues}, J. and {Levrier}, F. and {Lewis}, A. and {Liguori}, M. and {Lilje}, P.~B. and {Linden-V{\o}rnle}, M. and {L{\'o}pez-Caniego}, M. and {Lubin}, P.~M. and {Ma}, Y. -Z. and {Mac{\'\i}as-P{\'e}rez}, J.~F. and {Maggio}, G. and {Maino}, D. and {Mandolesi}, N. and {Mangilli}, A. and {Maris}, M. and {Martin}, P.~G. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Masi}, S. and {Matarrese}, S. and {McGehee}, P. and {Meinhold}, P.~R. and {Melchiorri}, A. and {Mendes}, L. and {Mennella}, A. and {Migliaccio}, M. and {Mitra}, S. and {Miville-Desch{\^e}nes}, M. -A. and {Molinari}, D. and {Moneti}, A. and {Montier}, L. and {Morgante}, G. and {Mortlock}, D. and {Moss}, A. and {M{\"u}nchmeyer}, M. and {Munshi}, D. and {Murphy}, J.~A. and {Naselsky}, P. and {Nati}, F. and {Natoli}, P. and {Netterfield}, C.~B. and {N{\o}rgaard-Nielsen}, H.~U. and {Noviello}, F. and {Novikov}, D. and {Novikov}, I. and {Oxborrow}, C.~A. and {Paci}, F. and {Pagano}, L. and {Pajot}, F. and {Paladini}, R. and {Pandolfi}, S. and {Paoletti}, D. and {Pasian}, F. and {Patanchon}, G. and {Pearson}, T.~J. and {Peiris}, H.~V. and {Perdereau}, O. and {Perotto}, L. and {Perrotta}, F. and {Pettorino}, V. and {Piacentini}, F. and {Piat}, M. and {Pierpaoli}, E. and {Pietrobon}, D. and {Plaszczynski}, S. and {Pointecouteau}, E. and {Polenta}, G. and {Popa}, L. and {Pratt}, G.~W. and {Pr{\'e}zeau}, G. and {Prunet}, S. and {Puget}, J. -L. and {Rachen}, J.~P. and {Reach}, W.~T. and {Rebolo}, R. and {Reinecke}, M. and {Remazeilles}, M. and {Renault}, C. and {Renzi}, A. and {Ristorcelli}, I. and {Rocha}, G. and {Rosset}, C. and {Rossetti}, M. and {Roudier}, G. and {Rowan-Robinson}, M. and {Rubi{\~n}o-Mart{\'\i}n}, J.~A. and {Rusholme}, B. and {Sandri}, M. and {Santos}, D. and {Savelainen}, M. and {Savini}, G. and {Scott}, D. and {Seiffert}, M.~D. and {Shellard}, E.~P.~S. and {Shiraishi}, M. and {Spencer}, L.~D. and {Stolyarov}, V. and {Stompor}, R. and {Sudiwala}, R. and {Sunyaev}, R. and {Sutton}, D. and {Suur-Uski}, A. -S. and {Sygnet}, J. -F. and {Tauber}, J.~A. and {Terenzi}, L. and {Toffolatti}, L. and {Tomasi}, M. and {Tristram}, M. and {Trombetti}, T. and {Tucci}, M. and {Tuovinen}, J. and {Valenziano}, L. and {Valiviita}, J. and {Van Tent}, B. and {Vielva}, P. and {Villa}, F. and {Wade}, L.~A. and {Wandelt}, B.~D. and {Wehus}, I.~K. and {White}, M. and {Yvon}, D. and {Zacchei}, A. and {Zibin}, J.~P. and {Zonca}, A.},
        title = "{Planck 2015 results. XX. Constraints on inflation}",
      journal = {\aap},
     keywords = {cosmic background radiation, cosmology: theory, early Universe, inflation, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2016,
        month = sep,
       volume = {594},
          eid = {A20},
        pages = {A20},
          doi = {10.1051/0004-6361/201525898},
archivePrefix = {arXiv},
       eprint = {1502.02114},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...594A..20P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{PlanckInflation18,
       author = {{Planck Collaboration} and {Akrami}, Y. and {Arroja}, F. and
         {Ashdown}, M. and {Aumont}, J. and {Baccigalupi}, C. and
         {Ballardini}, M. and {Banday}, A.~J. and {Barreiro}, R.~B. and
         {Bartolo}, N. and {Basak}, S. and {Benabed}, K. and {Bernard}, J. -P. and
         {Bersanelli}, M. and {Bielewicz}, P. and {Bock}, J.~J. and
         {Bond}, J.~R. and {Borrill}, J. and {Bouchet}, F.~R. and
         {Boulanger}, F. and {Bucher}, M. and {Burigana}, C. and
         {Butler}, R.~C. and {Calabrese}, E. and {Cardoso}, J. -F. and
         {Carron}, J. and {Challinor}, A. and {Chiang}, H.~C. and
         {Colombo}, L.~P.~L. and {Combet}, C. and {Contreras}, D. and
         {Crill}, B.~P. and {Cuttaia}, F. and {de Bernardis}, P. and
         {de Zotti}, G. and {Delabrouille}, J. and {Delouis}, J. -M. and
         {Di Valentino}, E. and {Diego}, J.~M. and {Donzelli}, S. and
         {Dor{\'e}}, O. and {Douspis}, M. and {Ducout}, A. and {Dupac}, X. and
         {Dusini}, S. and {Efstathiou}, G. and {Elsner}, F. and
         {En{\ss}lin}, T.~A. and {Eriksen}, H.~K. and {Fantaye}, Y. and
         {Fergusson}, J. and {Fernandez-Cobos}, R. and {Finelli}, F. and
         {Forastieri}, F. and {Frailis}, M. and {Franceschi}, E. and
         {Frolov}, A. and {Galeotta}, S. and {Galli}, S. and {Ganga}, K. and
         {Gauthier}, C. and {G{\'e}nova-Santos}, R.~T. and {Gerbino}, M. and
         {Ghosh}, T. and {Gonz{\'a}lez-Nuevo}, J. and {G{\'o}rski}, K.~M. and
         {Gratton}, S. and {Gruppuso}, A. and {Gudmundsson}, J.~E. and
         {Hamann}, J. and {Handley}, W. and {Hansen}, F.~K. and {Herranz}, D. and
         {Hivon}, E. and {Hooper}, D.~C. and {Huang}, Z. and {Jaffe}, A.~H. and
         {Jones}, W.~C. and {Keih{\"a}nen}, E. and {Keskitalo}, R. and
         {Kiiveri}, K. and {Kim}, J. and {Kisner}, T.~S. and
         {Krachmalnicoff}, N. and {Kunz}, M. and {Kurki-Suonio}, H. and
         {Lagache}, G. and {Lamarre}, J. -M. and {Lasenby}, A. and
         {Lattanzi}, M. and {Lawrence}, C.~R. and {Le Jeune}, M. and
         {Lesgourgues}, J. and {Levrier}, F. and {Lewis}, A. and {Liguori}, M. and
         {Lilje}, P.~B. and {Lindholm}, V. and {Lpez-Caniego}, M. and
         {Lubin}, P.~M. and {Ma}, Y. -Z. and {Mac{\'\i}as-P{\'e}rez}, J.~F. and
         {Maggio}, G. and {Maino}, D. and {Mandolesi}, N. and {Mangilli}, A. and
         {Marcos-Caballero}, A. and {Maris}, M. and {Martin}, P.~G. and
         {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Matarrese}, S. and {Mauri}, N. and
         {McEwen}, J.~D. and {Meerburg}, P.~D. and {Meinhold}, P.~R. and
         {Melchiorri}, A. and {Mennella}, A. and {Migliaccio}, M. and
         {Mitra}, S. and {Miville-Desch{\^e}nes}, M. -A. and {Molinari}, D. and
         {Moneti}, A. and {Montier}, L. and {Morgante}, G. and {Moss}, A. and
         {M{\"u}nchmeyer}, M. and {Natoli}, P. and {N{\o}rgaard-Nielsen}, H.~U. and
         {Pagano}, L. and {Paoletti}, D. and {Partridge}, B. and
         {Patanchon}, G. and {Peiris}, H.~V. and {Perrotta}, F. and
         {Pettorino}, V. and {Piacentini}, F. and {Polastri}, L. and
         {Polenta}, G. and {Puget}, J. -L. and {Rachen}, J.~P. and
         {Reinecke}, M. and {Remazeilles}, M. and {Renzi}, A. and {Rocha}, G. and
         {Rosset}, C. and {Roudier}, G. and {Rubi{\~n}o-Mart{\'\i}n}, J.~A. and
         {Ruiz-Granados}, B. and {Salvati}, L. and {Sandri}, M. and
         {Savelainen}, M. and {Scott}, D. and {Shellard}, E.~P.~S. and
         {Shiraishi}, M. and {Sirignano}, C. and {Sirri}, G. and
         {Spencer}, L.~D. and {Sunyaev}, R. and {Suur-Uski}, A. -S. and
         {Tauber}, J.~A. and {Tavagnacco}, D. and {Tenti}, M. and
         {Toffolatti}, L. and {Tomasi}, M. and {Trombetti}, T. and
         {Valiviita}, J. and {Van Tent}, B. and {Vielva}, P. and {Villa}, F. and
         {Vittorio}, N. and {Wandelt}, B.~D. and {Wehus}, I.~K. and
         {White}, S.~D.~M. and {Zacchei}, A. and {Zibin}, J.~P. and {Zonca}, A.},
        title = "{ 2018 results. X. Constraints on inflation}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2018,
        month = jul,
          eid = {arXiv:1807.06211},
        pages = {arXiv:1807.06211},
archivePrefix = {arXiv},
       eprint = {1807.06211},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018arXiv180706211P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{15Parameters,
       author = {{ Collaboration} and {Ade}, P.~A.~R. and {Aghanim}, N. and {Arnaud}, M. and {Ashdown}, M. and {Aumont}, J. and {Baccigalupi}, C. and {Banday}, A.~J. and {Barreiro}, R.~B. and {Bartlett}, J.~G. and {Bartolo}, N. and {Battaner}, E. and {Battye}, R. and {Benabed}, K. and {Beno{\^\i}t}, A. and {Benoit-L{\'e}vy}, A. and {Bernard}, J. -P. and {Bersanelli}, M. and {Bielewicz}, P. and {Bock}, J.~J. and {Bonaldi}, A. and {Bonavera}, L. and {Bond}, J.~R. and {Borrill}, J. and {Bouchet}, F.~R. and {Boulanger}, F. and {Bucher}, M. and {Burigana}, C. and {Butler}, R.~C. and {Calabrese}, E. and {Cardoso}, J. -F. and {Catalano}, A. and {Challinor}, A. and {Chamballu}, A. and {Chary}, R. -R. and {Chiang}, H.~C. and {Chluba}, J. and {Christensen}, P.~R. and {Church}, S. and {Clements}, D.~L. and {Colombi}, S. and {Colombo}, L.~P.~L. and {Combet}, C. and {Coulais}, A. and {Crill}, B.~P. and {Curto}, A. and {Cuttaia}, F. and {Danese}, L. and {Davies}, R.~D. and {Davis}, R.~J. and {de Bernardis}, P. and {de Rosa}, A. and {de Zotti}, G. and {Delabrouille}, J. and {D{\'e}sert}, F. -X. and {Di Valentino}, E. and {Dickinson}, C. and {Diego}, J.~M. and {Dolag}, K. and {Dole}, H. and {Donzelli}, S. and {Dor{\'e}}, O. and {Douspis}, M. and {Ducout}, A. and {Dunkley}, J. and {Dupac}, X. and {Efstathiou}, G. and {Elsner}, F. and {En{\ss}lin}, T.~A. and {Eriksen}, H.~K. and {Farhang}, M. and {Fergusson}, J. and {Finelli}, F. and {Forni}, O. and {Frailis}, M. and {Fraisse}, A.~A. and {Franceschi}, E. and {Frejsel}, A. and {Galeotta}, S. and {Galli}, S. and {Ganga}, K. and {Gauthier}, C. and {Gerbino}, M. and {Ghosh}, T. and {Giard}, M. and {Giraud-H{\'e}raud}, Y. and {Giusarma}, E. and {Gjerl{\o}w}, E. and {Gonz{\'a}lez-Nuevo}, J. and {G{\'o}rski}, K.~M. and {Gratton}, S. and {Gregorio}, A. and {Gruppuso}, A. and {Gudmundsson}, J.~E. and {Hamann}, J. and {Hansen}, F.~K. and {Hanson}, D. and {Harrison}, D.~L. and {Helou}, G. and {Henrot-Versill{\'e}}, S. and {Hern{\'a}ndez-Monteagudo}, C. and {Herranz}, D. and {Hildebrandt}, S.~R. and {Hivon}, E. and {Hobson}, M. and {Holmes}, W.~A. and {Hornstrup}, A. and {Hovest}, W. and {Huang}, Z. and {Huffenberger}, K.~M. and {Hurier}, G. and {Jaffe}, A.~H. and {Jaffe}, T.~R. and {Jones}, W.~C. and {Juvela}, M. and {Keih{\"a}nen}, E. and {Keskitalo}, R. and {Kisner}, T.~S. and {Kneissl}, R. and {Knoche}, J. and {Knox}, L. and {Kunz}, M. and {Kurki-Suonio}, H. and {Lagache}, G. and {L{\"a}hteenm{\"a}ki}, A. and {Lamarre}, J. -M. and {Lasenby}, A. and {Lattanzi}, M. and {Lawrence}, C.~R. and {Leahy}, J.~P. and {Leonardi}, R. and {Lesgourgues}, J. and {Levrier}, F. and {Lewis}, A. and {Liguori}, M. and {Lilje}, P.~B. and {Linden-V{\o}rnle}, M. and {L{\'o}pez-Caniego}, M. and {Lubin}, P.~M. and {Mac{\'\i}as-P{\'e}rez}, J.~F. and {Maggio}, G. and {Maino}, D. and {Mandolesi}, N. and {Mangilli}, A. and {Marchini}, A. and {Maris}, M. and {Martin}, P.~G. and {Martinelli}, M. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Masi}, S. and {Matarrese}, S. and {McGehee}, P. and {Meinhold}, P.~R. and {Melchiorri}, A. and {Melin}, J. -B. and {Mendes}, L. and {Mennella}, A. and {Migliaccio}, M. and {Millea}, M. and {Mitra}, S. and {Miville-Desch{\^e}nes}, M. -A. and {Moneti}, A. and {Montier}, L. and {Morgante}, G. and {Mortlock}, D. and {Moss}, A. and {Munshi}, D. and {Murphy}, J.~A. and {Naselsky}, P. and {Nati}, F. and {Natoli}, P. and {Netterfield}, C.~B. and {N{\o}rgaard-Nielsen}, H.~U. and {Noviello}, F. and {Novikov}, D. and {Novikov}, I. and {Oxborrow}, C.~A. and {Paci}, F. and {Pagano}, L. and {Pajot}, F. and {Paladini}, R. and {Paoletti}, D. and {Partridge}, B. and {Pasian}, F. and {Patanchon}, G. and {Pearson}, T.~J. and {Perdereau}, O. and {Perotto}, L. and {Perrotta}, F. and {Pettorino}, V. and {Piacentini}, F. and {Piat}, M. and {Pierpaoli}, E. and {Pietrobon}, D. and {Plaszczynski}, S. and {Pointecouteau}, E. and {Polenta}, G. and {Popa}, L. and {Pratt}, G.~W. and {Pr{\'e}zeau}, G. and {Prunet}, S. and {Puget}, J. -L. and {Rachen}, J.~P. and {Reach}, W.~T. and {Rebolo}, R. and {Reinecke}, M. and {Remazeilles}, M. and {Renault}, C. and {Renzi}, A. and {Ristorcelli}, I. and {Rocha}, G. and {Rosset}, C. and {Rossetti}, M. and {Roudier}, G. and {Rouill{\'e} d'Orfeuil}, B. and {Rowan-Robinson}, M. and {Rubi{\~n}o-Mart{\'\i}n}, J.~A. and {Rusholme}, B. and {Said}, N. and {Salvatelli}, V. and {Salvati}, L. and {Sandri}, M. and {Santos}, D. and {Savelainen}, M. and {Savini}, G. and {Scott}, D. and {Seiffert}, M.~D. and {Serra}, P. and {Shellard}, E.~P.~S. and {Spencer}, L.~D. and {Spinelli}, M. and {Stolyarov}, V. and {Stompor}, R. and {Sudiwala}, R. and {Sunyaev}, R. and {Sutton}, D. and {Suur-Uski}, A. -S. and {Sygnet}, J. -F. and {Tauber}, J.~A. and {Terenzi}, L. and {Toffolatti}, L. and {Tomasi}, M. and {Tristram}, M. and {Trombetti}, T. and {Tucci}, M. and {Tuovinen}, J. and {T{\"u}rler}, M. and {Umana}, G. and {Valenziano}, L. and {Valiviita}, J. and {Van Tent}, F. and {Vielva}, P. and {Villa}, F. and {Wade}, L.~A. and {Wandelt}, B.~D. and {Wehus}, I.~K. and {White}, M. and {White}, S.~D.~M. and {Wilkinson}, A. and {Yvon}, D. and {Zacchei}, A. and {Zonca}, A.},
        title = "{ 2015 results. XIII. Cosmological parameters}",
      journal = {\aap},
     keywords = {cosmology: observations, cosmology: theory, cosmic background radiation, cosmological parameters, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2016,
        month = sep,
       volume = {594},
          eid = {A13},
        pages = {A13},
          doi = {10.1051/0004-6361/201525830},
archivePrefix = {arXiv},
       eprint = {1502.01589},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...594A..13P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{18Parameters,
       author = {{ Collaboration} and {Aghanim}, N. and {Akrami}, Y. and {Ashdown}, M. and {Aumont}, J. and {Baccigalupi}, C. and {Ballardini}, M. and {Banday}, A.~J. and {Barreiro}, R.~B. and {Bartolo}, N. and {Basak}, S. and {Battye}, R. and {Benabed}, K. and {Bernard}, J. -P. and {Bersanelli}, M. and {Bielewicz}, P. and {Bock}, J.~J. and {Bond}, J.~R. and {Borrill}, J. and {Bouchet}, F.~R. and {Boulanger}, F. and {Bucher}, M. and {Burigana}, C. and {Butler}, R.~C. and {Calabrese}, E. and {Cardoso}, J. -F. and {Carron}, J. and {Challinor}, A. and {Chiang}, H.~C. and {Chluba}, J. and {Colombo}, L.~P.~L. and {Combet}, C. and {Contreras}, D. and {Crill}, B.~P. and {Cuttaia}, F. and {de Bernardis}, P. and {de Zotti}, G. and {Delabrouille}, J. and {Delouis}, J. -M. and {Di Valentino}, E. and {Diego}, J.~M. and {Dor{\'e}}, O. and {Douspis}, M. and {Ducout}, A. and {Dupac}, X. and {Dusini}, S. and {Efstathiou}, G. and {Elsner}, F. and {En{\ss}lin}, T.~A. and {Eriksen}, H.~K. and {Fantaye}, Y. and {Farhang}, M. and {Fergusson}, J. and {Fernandez-Cobos}, R. and {Finelli}, F. and {Forastieri}, F. and {Frailis}, M. and {Fraisse}, A.~A. and {Franceschi}, E. and {Frolov}, A. and {Galeotta}, S. and {Galli}, S. and {Ganga}, K. and {G{\'e}nova-Santos}, R.~T. and {Gerbino}, M. and {Ghosh}, T. and {Gonz{\'a}lez-Nuevo}, J. and {G{\'o}rski}, K.~M. and {Gratton}, S. and {Gruppuso}, A. and {Gudmundsson}, J.~E. and {Hamann}, J. and {Handley}, W. and {Hansen}, F.~K. and {Herranz}, D. and {Hildebrandt}, S.~R. and {Hivon}, E. and {Huang}, Z. and {Jaffe}, A.~H. and {Jones}, W.~C. and {Karakci}, A. and {Keih{\"a}nen}, E. and {Keskitalo}, R. and {Kiiveri}, K. and {Kim}, J. and {Kisner}, T.~S. and {Knox}, L. and {Krachmalnicoff}, N. and {Kunz}, M. and {Kurki-Suonio}, H. and {Lagache}, G. and {Lamarre}, J. -M. and {Lasenby}, A. and {Lattanzi}, M. and {Lawrence}, C.~R. and {Le Jeune}, M. and {Lemos}, P. and {Lesgourgues}, J. and {Levrier}, F. and {Lewis}, A. and {Liguori}, M. and {Lilje}, P.~B. and {Lilley}, M. and {Lindholm}, V. and {L{\'o}pez-Caniego}, M. and {Lubin}, P.~M. and {Ma}, Y. -Z. and {Mac{\'\i}as-P{\'e}rez}, J.~F. and {Maggio}, G. and {Maino}, D. and {Mandolesi}, N. and {Mangilli}, A. and {Marcos-Caballero}, A. and {Maris}, M. and {Martin}, P.~G. and {Martinelli}, M. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Matarrese}, S. and {Mauri}, N. and {McEwen}, J.~D. and {Meinhold}, P.~R. and {Melchiorri}, A. and {Mennella}, A. and {Migliaccio}, M. and {Millea}, M. and {Mitra}, S. and {Miville-Desch{\^e}nes}, M. -A. and {Molinari}, D. and {Montier}, L. and {Morgante}, G. and {Moss}, A. and {Natoli}, P. and {N{\o}rgaard-Nielsen}, H.~U. and {Pagano}, L. and {Paoletti}, D. and {Partridge}, B. and {Patanchon}, G. and {Peiris}, H.~V. and {Perrotta}, F. and {Pettorino}, V. and {Piacentini}, F. and {Polastri}, L. and {Polenta}, G. and {Puget}, J. -L. and {Rachen}, J.~P. and {Reinecke}, M. and {Remazeilles}, M. and {Renzi}, A. and {Rocha}, G. and {Rosset}, C. and {Roudier}, G. and {Rubi{\~n}o-Mart{\'\i}n}, J.~A. and {Ruiz-Granados}, B. and {Salvati}, L. and {Sandri}, M. and {Savelainen}, M. and {Scott}, D. and {Shellard}, E.~P.~S. and {Sirignano}, C. and {Sirri}, G. and {Spencer}, L.~D. and {Sunyaev}, R. and {Suur-Uski}, A. -S. and {Tauber}, J.~A. and {Tavagnacco}, D. and {Tenti}, M. and {Toffolatti}, L. and {Tomasi}, M. and {Trombetti}, T. and {Valenziano}, L. and {Valiviita}, J. and {Van Tent}, B. and {Vibert}, L. and {Vielva}, P. and {Villa}, F. and {Vittorio}, N. and {Wandelt}, B.~D. and {Wehus}, I.~K. and {White}, M. and {White}, S.~D.~M. and {Zacchei}, A. and {Zonca}, A.},
        title = "{ 2018 results. VI. Cosmological parameters}",
      journal = {\aap},
     keywords = {cosmic background radiation, cosmological parameters, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = sep,
       volume = {641},
          eid = {A6},
        pages = {A6},
          doi = {10.1051/0004-6361/201833910},
archivePrefix = {arXiv},
       eprint = {1807.06209},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...641A...6P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{MandatoryPolyChord1,
       author = {{Handley}, W.~J. and {Hobson}, M.~P. and {Lasenby}, A.~N.},
        title = "{polychord: nested sampling for cosmology.}",
      journal = {\mnras},
     keywords = {methods: data analysis, methods: statistical, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2015,
        month = jun,
       volume = {450},
        pages = {L61-L65},
          doi = {10.1093/mnrasl/slv047},
archivePrefix = {arXiv},
       eprint = {1502.01856},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.450L..61H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{MandatoryPolyChord2,
       author = {{Handley}, W.~J. and {Hobson}, M.~P. and {Lasenby}, A.~N.},
        title = "{POLYCHORD: next-generation nested sampling}",
      journal = {\mnras},
     keywords = {methods: data analysis, methods: statistical, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2015,
        month = nov,
       volume = {453},
       number = {4},
        pages = {4384-4398},
          doi = {10.1093/mnras/stv1911},
archivePrefix = {arXiv},
       eprint = {1506.00171},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.453.4384H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ag14,
       author = {{Cole}, Shaun and {Percival}, Will J. and {Peacock}, John A. and
         {Norberg}, Peder and {Baugh}, Carlton M. and {Frenk}, Carlos S. and
         {Baldry}, Ivan and {Bland-Hawthorn}, Joss and {Bridges}, Terry and
         {Cannon}, Russell and {Colless}, Matthew and {Collins}, Chris and
         {Couch}, Warrick and {Cross}, Nicholas J.~G. and {Dalton}, Gavin and
         {Eke}, Vincent R. and {De Propris}, Roberto and {Driver}, Simon P. and
         {Efstathiou}, George and {Ellis}, Richard S. and {Glazebrook}, Karl and
         {Jackson}, Carole and {Jenkins}, Adrian and {Lahav}, Ofer and
         {Lewis}, Ian and {Lumsden}, Stuart and {Maddox}, Steve and
         {Madgwick}, Darren and {Peterson}, Bruce A. and {Sutherland}, Will and
         {Taylor}, Keith},
        title = "{The 2dF Galaxy Redshift Survey: power-spectrum analysis of the final data set and cosmological implications}",
      journal = {\mnras},
     keywords = {cosmological parameters, large-scale structure of Universe, Astrophysics},
         year = 2005,
        month = sep,
       volume = {362},
       number = {2},
        pages = {505-534},
          doi = {10.1111/j.1365-2966.2005.09318.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0501174},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005MNRAS.362..505C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{QnlAg,
       author = {{Seljak}, Uros and {Slosar}, Anze and {McDonald}, Patrick},
        title = "{Cosmological parameters from combining the Lyman-{\ensuremath{\alpha}} forest with CMB, galaxy clustering and SN constraints}",
      journal = {\jcap},
     keywords = {Astrophysics, High Energy Physics - Phenomenology},
         year = 2006,
        month = oct,
       volume = {2006},
       number = {10},
          eid = {014},
        pages = {014},
          doi = {10.1088/1475-7516/2006/10/014},
archivePrefix = {arXiv},
       eprint = {astro-ph/0604335},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006JCAP...10..014S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{WMAP3,
       author = {{Spergel}, D.~N. and {Bean}, R. and {Dor{\'e}}, O. and {Nolta}, M.~R. and
         {Bennett}, C.~L. and {Dunkley}, J. and {Hinshaw}, G. and {Jarosik}, N. and
         {Komatsu}, E. and {Page}, L. and {Peiris}, H.~V. and {Verde}, L. and
         {Halpern}, M. and {Hill}, R.~S. and {Kogut}, A. and {Limon}, M. and
         {Meyer}, S.~S. and {Odegard}, N. and {Tucker}, G.~S. and {Weiland
        }, J.~L. and {Wollack}, E. and {Wright}, E.~L.},
        title = "{Three-Year Wilkinson Microwave Anisotropy Probe (WMAP) Observations: Implications for Cosmology}",
      journal = {\apjs},
     keywords = {Cosmology: Cosmic Microwave Background, Cosmology: Observations, Astrophysics},
         year = 2007,
        month = jun,
       volume = {170},
       number = {2},
        pages = {377-408},
          doi = {10.1086/513700},
archivePrefix = {arXiv},
       eprint = {astro-ph/0603449},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJS..170..377S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{RoyMcDonald2009,
       author = {{McDonald}, Patrick and {Roy}, Arabindo},
        title = "{Clustering of dark matter tracers: generalizing bias for the coming era of precision LSS}",
      journal = {\jcap},
     keywords = {Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2009,
        month = aug,
       volume = {2009},
       number = {8},
          eid = {020},
        pages = {020},
          doi = {10.1088/1475-7516/2009/08/020},
archivePrefix = {arXiv},
       eprint = {0902.0991},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009JCAP...08..020M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{APEffect,
       author = {{Beutler}, Florian and {Saito}, Shun and {Seo}, Hee-Jong and {Brinkmann}, Jon and {Dawson}, Kyle S. and {Eisenstein}, Daniel J. and {Font-Ribera}, Andreu and {Ho}, Shirley and {McBride}, Cameron K. and {Montesano}, Francesco and {Percival}, Will J. and {Ross}, Ashley J. and {Ross}, Nicholas P. and {Samushia}, Lado and {Schlegel}, David J. and {S{\'a}nchez}, Ariel G. and {Tinker}, Jeremy L. and {Weaver}, Benjamin A.},
        title = "{The clustering of galaxies in the SDSS-III Baryon Oscillation Spectroscopic Survey: testing gravity with redshift space distortions using the power spectrum multipoles}",
      journal = {\mnras},
     keywords = {gravitation, surveys, cosmological parameters, cosmology: observations, dark energy, large-scale structure of Universe, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2014,
        month = sep,
       volume = {443},
       number = {2},
        pages = {1065-1089},
          doi = {10.1093/mnras/stu1051},
archivePrefix = {arXiv},
       eprint = {1312.4611},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.443.1065B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{BOSSDR11,
       author = {{Gil-Mar{\'\i}n}, H{\'e}ctor and {Nore{\~n}a}, Jorge and {Verde}, Licia and {Percival}, Will J. and {Wagner}, Christian and {Manera}, Marc and {Schneider}, Donald P.},
        title = "{The power spectrum and bispectrum of SDSS DR11 BOSS galaxies - I. Bias and gravity}",
      journal = {\mnras},
     keywords = {galaxies: haloes, cosmological parameters, cosmology: theory, large-scale structure of Universe, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = jul,
       volume = {451},
       number = {1},
        pages = {539-580},
          doi = {10.1093/mnras/stv961},
archivePrefix = {arXiv},
       eprint = {1407.5668},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.451..539G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{BOSSDR12,
       author = {{Gil-Mar{\'\i}n}, H{\'e}ctor and {Percival}, Will J. and
         {Brownstein}, Joel R. and {Chuang}, Chia-Hsun and {Grieb}, Jan Niklas and
         {Ho}, Shirley and {Kitaura}, Francisco-Shu and {Maraston}, Claudia and
         {Prada}, Francisco and {Rodr{\'\i}guez-Torres}, Sergio and
         {Ross}, Ashley J. and {Samushia}, Lado and {Schlegel}, David J. and
         {Thomas}, Daniel and {Tinker}, Jeremy L. and {Zhao}, Gong-Bo},
        title = "{The clustering of galaxies in the SDSS-III Baryon Oscillation Spectroscopic Survey: RSD measurement from the LOS-dependent power spectrum of DR12 BOSS galaxies}",
      journal = {\mnras},
     keywords = {galaxies: haloes, cosmological parameters, cosmology: theory, large-scale structure of Universe, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2016,
        month = aug,
       volume = {460},
       number = {4},
        pages = {4188-4209},
          doi = {10.1093/mnras/stw1096},
archivePrefix = {arXiv},
       eprint = {1509.06386},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.460.4188G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{TNS1,
  title = {Baryon acoustic oscillations in 2D: Modeling redshift-space power spectrum from perturbation theory},
  author = {Taruya, Atsushi and Nishimichi, Takahiro and Saito, Shun},
  journal = {Phys. Rev. D},
  volume = {82},
  issue = {6},
  pages = {063522},
  numpages = {18},
  year = {2010},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.82.063522},
  url = {https://link.aps.org/doi/10.1103/PhysRevD.82.063522}
}



@article{TNS2,
  title = {Baryon acoustic oscillations in 2D. II. Redshift-space halo clustering in $N$-body simulations},
  author = {Nishimichi, Takahiro and Taruya, Atsushi},
  journal = {Phys. Rev. D},
  volume = {84},
  issue = {4},
  pages = {043526},
  numpages = {15},
  year = {2011},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.84.043526},
  url = {https://link.aps.org/doi/10.1103/PhysRevD.84.043526}
}

@ARTICLE{APEffectHistorico,
       author = {{Alcock}, C. and {Paczynski}, B.},
        title = "{An evolution free test for non-zero cosmological constant}",
      journal = {\nat},
     keywords = {Astrophysics},
         year = 1979,
        month = oct,
       volume = {281},
        pages = {358},
          doi = {10.1038/281358a0},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1979Natur.281..358A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{RescoMaroto,
       author = {{Aparicio Resco}, Miguel and {Maroto}, Antonio L. and {Alcaniz}, Jailson S. and {Abramo}, L. Raul and {Hern{\'a}ndez-Monteagudo}, C. and {Ben{\'\i}tez}, N. and {Carneiro}, S. and {Cenarro}, A.~J. and {Crist{\'o}bal-Hornillos}, D. and {Dupke}, R.~A. and {Ederoclite}, A. and {L{\'o}pez-Sanjuan}, C. and {Mar{\'\i}n-Franch}, A. and {Moles}, M. and {Oliveira}, C.~M. and {Sodr{\'e}}, L., Jr. and {Taylor}, K. and {Varela}, J. and {V{\'a}zquez Rami{\'o}}, H.},
        title = "{J-PAS: forecasts on dark energy and modified gravity theories}",
      journal = {\mnras},
     keywords = {dark energy, large-scale structure of Universe, Astrophysics - Cosmology and Nongalactic Astrophysics, General Relativity and Quantum Cosmology},
         year = 2020,
        month = apr,
       volume = {493},
       number = {3},
        pages = {3616-3631},
          doi = {10.1093/mnras/staa367},
archivePrefix = {arXiv},
       eprint = {1910.02694},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.493.3616A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{MirandaHuModeloFeature,
       author = {{Miranda}, Vin{\'\i}cius and {Hu}, Wayne},
        title = "{Inflationary steps in the Planck data}",
      journal = {\prd},
     keywords = {98.80.Cq, 98.70.Vc, Particle-theory and field-theory models of the early Universe, Background radiations, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2014,
        month = apr,
       volume = {89},
       number = {8},
          eid = {083529},
        pages = {083529},
          doi = {10.1103/PhysRevD.89.083529},
archivePrefix = {arXiv},
       eprint = {1312.0946},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014PhRvD..89h3529M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CC1NeutrinosModel,
       author = {{Choudhury}, Shouvik Roy and {Hannestad}, Steen and {Tram}, Thomas},
        title = "{Massive neutrino self-interactions and Inflation}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, High Energy Physics - Phenomenology},
         year = 2022,
        month = jul,
          eid = {arXiv:2207.07142},
        pages = {arXiv:2207.07142},
archivePrefix = {arXiv},
       eprint = {2207.07142},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022arXiv220707142C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CC2ConstraintsCMB,
       author = {{Hazra}, Dhiraj Kumar and {Paoletti}, Daniela and {Debono}, Ivan and {Shafieloo}, Arman and {Smoot}, George F. and {Starobinsky}, Alexei A.},
        title = "{Inflation story: slow-roll and beyond}",
      journal = {\jcap},
     keywords = {inflation, Inflation and CMBR theory, non-gaussianity, Astrophysics - Cosmology and Nongalactic Astrophysics, High Energy Physics - Phenomenology, High Energy Physics - Theory},
         year = 2021,
        month = dec,
       volume = {2021},
       number = {12},
          eid = {038},
        pages = {038},
          doi = {10.1088/1475-7516/2021/12/038},
archivePrefix = {arXiv},
       eprint = {2107.09460},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021JCAP...12..038H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CC3TwoFieldComparison,
       author = {{Braglia}, Matteo and {Chen}, Xingang and {Hazra}, Dhiraj Kumar},
        title = "{Comparing multi-field primordial feature models with the Planck data}",
      journal = {\jcap},
     keywords = {cosmological parameters from CMBR, cosmological perturbation theory, inflation, Astrophysics - Cosmology and Nongalactic Astrophysics, General Relativity and Quantum Cosmology, High Energy Physics - Phenomenology, High Energy Physics - Theory},
         year = 2021,
        month = jun,
       volume = {2021},
       number = {6},
          eid = {005},
        pages = {005},
          doi = {10.1088/1475-7516/2021/06/005},
archivePrefix = {arXiv},
       eprint = {2103.03025},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021JCAP...06..005B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CC4EarlierRecombination,
       author = {{Sekiguchi}, Toyokazu and {Takahashi}, Tomo},
        title = "{Early recombination as a solution to the H$_{0}$ tension}",
      journal = {\prd},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, General Relativity and Quantum Cosmology, High Energy Physics - Phenomenology},
         year = 2021,
        month = apr,
       volume = {103},
       number = {8},
          eid = {083507},
        pages = {083507},
          doi = {10.1103/PhysRevD.103.083507},
archivePrefix = {arXiv},
       eprint = {2007.03381},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021PhRvD.103h3507S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CC5NeutrinoConstraints,
       author = {{Choudhury}, Shouvik Roy and {Hannestad}, Steen and {Tram}, Thomas},
        title = "{Updated constraints on massive neutrino self-interactions from cosmology in light of the H$_{0}$ tension}",
      journal = {\jcap},
     keywords = {cosmological neutrinos, cosmological parameters from CMBR, neutrino masses from cosmology, cosmological perturbation theory, Astrophysics - Cosmology and Nongalactic Astrophysics, High Energy Physics - Phenomenology},
         year = 2021,
        month = mar,
       volume = {2021},
       number = {3},
          eid = {084},
        pages = {084},
          doi = {10.1088/1475-7516/2021/03/084},
archivePrefix = {arXiv},
       eprint = {2012.07519},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021JCAP...03..084C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CC6NeutrinoMasses,
       author = {{Choudhury}, Shouvik Roy and {Hannestad}, Steen},
        title = "{Updated results on neutrino mass and mass hierarchy from cosmology with Planck 2018 likelihoods}",
      journal = {\jcap},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, High Energy Physics - Experiment, High Energy Physics - Phenomenology},
         year = 2020,
        month = jul,
       volume = {2020},
       number = {7},
          eid = {037},
        pages = {037},
          doi = {10.1088/1475-7516/2020/07/037},
archivePrefix = {arXiv},
       eprint = {1907.12598},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020JCAP...07..037C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CC7DecelerationReconstructions,
       author = {{Xu}, Bing and {Xia}, Li-Xin},
        title = "{Reconstructing the evolution of deceleration parameter with the non-parametric Bayesian method}",
      journal = {\apss},
     keywords = {Cosmology, Cosmic acceleration, Deceleration parameter},
         year = 2020,
        month = feb,
       volume = {365},
       number = {2},
          eid = {44},
        pages = {44},
          doi = {10.1007/s10509-020-03755-z},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020Ap&SS.365...44X},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CC8DESSHOESBOSSTensions,
       author = {{Handley}, Will and {Lemos}, Pablo},
        title = "{Quantifying tensions in cosmological parameters: Interpreting the DES evidence ratio}",
      journal = {\prd},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2019,
        month = aug,
       volume = {100},
       number = {4},
          eid = {043504},
        pages = {043504},
          doi = {10.1103/PhysRevD.100.043504},
archivePrefix = {arXiv},
       eprint = {1902.04029},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019PhRvD.100d3504H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CC9Dimensionality,
       author = {{Handley}, Will and {Lemos}, Pablo},
        title = "{Quantifying dimensionality: Bayesian cosmological model complexities}",
      journal = {\prd},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2019,
        month = jul,
       volume = {100},
       number = {2},
          eid = {023512},
        pages = {023512},
          doi = {10.1103/PhysRevD.100.023512},
archivePrefix = {arXiv},
       eprint = {1903.06682},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019PhRvD.100b3512H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CC10Kinetic,
       author = {{Hergt}, L.~T. and {Handley}, W.~J. and {Hobson}, M.~P. and {Lasenby}, A.~N.},
        title = "{Constraining the kinetically dominated universe}",
      journal = {\prd},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, General Relativity and Quantum Cosmology},
         year = 2019,
        month = jul,
       volume = {100},
       number = {2},
          eid = {023501},
        pages = {023501},
          doi = {10.1103/PhysRevD.100.023501},
archivePrefix = {arXiv},
       eprint = {1809.07737},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019PhRvD.100b3501H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CC11NeutrinoSterile,
       author = {{Knee}, Alan M. and {Contreras}, Dagoberto and {Scott}, Douglas},
        title = "{Cosmological constraints on sterile neutrino oscillations from Planck}",
      journal = {\jcap},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, High Energy Physics - Experiment},
         year = 2019,
        month = jul,
       volume = {2019},
       number = {7},
          eid = {039},
        pages = {039},
          doi = {10.1088/1475-7516/2019/07/039},
archivePrefix = {arXiv},
       eprint = {1812.02102},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019JCAP...07..039K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CC12OsciBispectrum,
       author = {{Torrado}, Jes{\'u}s and {Hu}, Bin and {Ach{\'u}carro}, Ana},
        title = "{Robust predictions for an oscillatory bispectrum in Planck 2015 data from transient reductions in the speed of sound of the inflaton}",
      journal = {\prd},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2017,
        month = oct,
       volume = {96},
       number = {8},
          eid = {083515},
        pages = {083515},
          doi = {10.1103/PhysRevD.96.083515},
archivePrefix = {arXiv},
       eprint = {1611.10350},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017PhRvD..96h3515T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CC13TelescopePlanck,
       author = {{Joudaki}, Shahab and {Blake}, Chris and {Heymans}, Catherine and {Choi}, Ami and {Harnois-Deraps}, Joachim and {Hildebrandt}, Hendrik and {Joachimi}, Benjamin and {Johnson}, Andrew and {Mead}, Alexander and {Parkinson}, David and {Viola}, Massimo and {van Waerbeke}, Ludovic},
        title = "{CFHTLenS revisited: assessing concordance with Planck including astrophysical systematics}",
      journal = {\mnras},
     keywords = {gravitational lensing: weak, surveys, cosmology: theory, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2017,
        month = feb,
       volume = {465},
       number = {2},
        pages = {2033-2052},
          doi = {10.1093/mnras/stw2665},
archivePrefix = {arXiv},
       eprint = {1601.05786},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.465.2033J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CC14Qderivatives,
       author = {{Calcagni}, Gianluca and {Kuroyanagi}, Sachiko and {Tsujikawa}, Shinji},
        title = "{Cosmic microwave background and inflation in multi-fractional spacetimes}",
      journal = {\jcap},
     keywords = {High Energy Physics - Theory, Astrophysics - Cosmology and Nongalactic Astrophysics, General Relativity and Quantum Cosmology},
         year = 2016,
        month = aug,
       volume = {2016},
       number = {8},
          eid = {039},
        pages = {039},
          doi = {10.1088/1475-7516/2016/08/039},
archivePrefix = {arXiv},
       eprint = {1606.08449},
 primaryClass = {hep-th},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016JCAP...08..039C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CC15ThreeDarkEnergy,
       author = {{Zhang}, Hongchao and {Li}, Enkun and {Xu}, Lixin},
        title = "{Distinguish three time-dependent dark energy models using statefinder pairs with error bars and Bayesian evidence}",
      journal = {arXiv e-prints},
     keywords = {General Relativity and Quantum Cosmology, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2016,
        month = may,
          eid = {arXiv:1605.00213},
        pages = {arXiv:1605.00213},
archivePrefix = {arXiv},
       eprint = {1605.00213},
 primaryClass = {gr-qc},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016arXiv160500213Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ReconCMBWeakLensin,
       author = {{Chandra}, Rajorshi Sushovan and {Souradeep}, Tarun},
        title = "{Primordial Power Spectrum reconstruction from CMB Weak Lensing Power Spectrum}",
      journal = {\jcap},
     keywords = {CMBR theory, cosmological parameters from CMBR, gravitational lensing, inflation},
         year = 2021,
        month = oct,
       volume = {2021},
       number = {10},
          eid = {081},
        pages = {081},
          doi = {10.1088/1475-7516/2021/10/081},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021JCAP...10..081C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ReconLSSOrthogonal,
       author = {{Esmaeilian}, Muhammad Sadegh and {Farhang}, Marzieh and {Khodabakhshi}, Shirin},
        title = "{Detectable Data-driven Features in the Primordial Scalar Power Spectrum}",
      journal = {\apj},
     keywords = {Large-scale structure of the universe, Computational astronomy, Origin of the universe, Cosmic microwave background radiation, 902, 293, 1186, 322, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = may,
       volume = {912},
       number = {2},
          eid = {104},
        pages = {104},
          doi = {10.3847/1538-4357/abe865},
archivePrefix = {arXiv},
       eprint = {2011.14774},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...912..104E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ReconTopHat,
       author = {{Brando}, Guilherme and {Linder}, Eric V.},
        title = "{Exploring early and late cosmology with next generation surveys}",
      journal = {\prd},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = may,
       volume = {101},
       number = {10},
          eid = {103510},
        pages = {103510},
          doi = {10.1103/PhysRevD.101.103510},
archivePrefix = {arXiv},
       eprint = {2001.07738},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020PhRvD.101j3510B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{ReconSplines,
       author = {{Ravenni}, Andrea and {Verde}, Licia and {Cuesta}, Antonio J.},
        title = "{Red, Straight, no bends: primordial power spectrum reconstruction from CMB and large-scale structure}",
      journal = {\jcap},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, 85A40},
         year = 2016,
        month = aug,
       volume = {2016},
       number = {8},
          eid = {028},
        pages = {028},
          doi = {10.1088/1475-7516/2016/08/028},
archivePrefix = {arXiv},
       eprint = {1605.06637},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016JCAP...08..028R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ReconFilter,
       author = {{Dorn}, Sebastian and {Ramirez}, Erandy and {Kunze}, Kerstin E. and {Hofmann}, Stefan and {En{\ss}lin}, Torsten A.},
        title = "{Generic inference of inflation models by non-Gaussianity and primordial power spectrum reconstruction}",
      journal = {\jcap},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2014,
        month = jun,
       volume = {2014},
       number = {6},
          eid = {048},
        pages = {048},
          doi = {10.1088/1475-7516/2014/06/048},
archivePrefix = {arXiv},
       eprint = {1403.5067},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014JCAP...06..048D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ReconPRISM,
       author = {{Paykari}, P. and {Lanusse}, F. and {Starck}, J. -L. and {Sureau}, F. and {Bobin}, J.},
        title = "{PRISM: Sparse recovery of the primordial power spectrum}",
      journal = {\aap},
     keywords = {methods: statistical, cosmic background radiation, early Universe, inflation, methods: data analysis, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2014,
        month = jun,
       volume = {566},
          eid = {A77},
        pages = {A77},
          doi = {10.1051/0004-6361/201322326},
archivePrefix = {arXiv},
       eprint = {1402.1983},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014A&A...566A..77P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{InverseScalarDynamics,
       author = {{Kumazaki}, Kohei and {Yokoyama}, Shuichiro and {Sugiyama}, Naoshi},
        title = "{Fine features in the primordial power spectrum}",
      journal = {\jcap},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, General Relativity and Quantum Cosmology, High Energy Physics - Phenomenology, High Energy Physics - Theory},
         year = 2011,
        month = dec,
       volume = {2011},
       number = {12},
          eid = {008},
        pages = {008},
          doi = {10.1088/1475-7516/2011/12/008},
archivePrefix = {arXiv},
       eprint = {1105.2398},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011JCAP...12..008K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ReconSplinesWMAP3,
       author = {{Verde}, Licia and {Peiris}, Hiranya},
        title = "{On minimally parametric primordial power spectrum reconstruction and the evidence for a red tilt}",
      journal = {\jcap},
     keywords = {Astrophysics},
         year = 2008,
        month = jul,
       volume = {2008},
       number = {7},
          eid = {009},
        pages = {009},
          doi = {10.1088/1475-7516/2008/07/009},
archivePrefix = {arXiv},
       eprint = {0802.1219},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008JCAP...07..009V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ReconWaveletSimulated,
       author = {{Mukherjee}, Pia and {Wang}, Yun},
        title = "{Primordial power spectrum reconstruction}",
      journal = {\jcap},
     keywords = {Astrophysics},
         year = 2005,
        month = dec,
       volume = {2005},
       number = {12},
          eid = {007},
        pages = {007},
          doi = {10.1088/1475-7516/2005/12/007},
archivePrefix = {arXiv},
       eprint = {astro-ph/0502136},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005JCAP...12..007M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ReconWaveletReal,
       author = {{Mukherjee}, Pia and {Wang}, Yun},
        title = "{Direct Wavelet Expansion of the Primordial Power Spectrum}",
      journal = {\apj},
     keywords = {Cosmology: Cosmic Microwave Background, Cosmology: Early Universe, Methods: Numerical, Astrophysics, High Energy Physics - Phenomenology},
         year = 2003,
        month = dec,
       volume = {598},
       number = {2},
        pages = {779-784},
          doi = {10.1086/379107},
archivePrefix = {arXiv},
       eprint = {astro-ph/0301562},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003ApJ...598..779M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ReconSplinesWMAP1,
       author = {{Sealfon}, Carolyn and {Verde}, Licia and {Jimenez}, Raul},
        title = "{Smoothing spline primordial power spectrum reconstruction}",
      journal = {\prd},
     keywords = {98.80.Es, Observational cosmology, Astrophysics},
         year = 2005,
        month = nov,
       volume = {72},
       number = {10},
          eid = {103520},
        pages = {103520},
          doi = {10.1103/PhysRevD.72.103520},
archivePrefix = {arXiv},
       eprint = {astro-ph/0506707},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005PhRvD..72j3520S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Starobinski1979,
       author = {{Starobinski{\v{i}}}, A.~A.},
        title = "{Spectrum of relict gravitational radiation and the early state of the universe}",
      journal = {Soviet Journal of Experimental and Theoretical Physics Letters},
         year = 1979,
        month = dec,
       volume = {30},
        pages = {682},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1979JETPL..30..682S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Linde1982,
       author = {{Linde}, A.~D.},
        title = "{A new inflationary universe scenario: A possible solution of the horizon, flatness, homogeneity, isotropy and primordial monopole problems}",
      journal = {Physics Letters B},
         year = 1982,
        month = feb,
       volume = {108},
       number = {6},
        pages = {389-393},
          doi = {10.1016/0370-2693(82)91219-9},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1982PhLB..108..389L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{SearchingFeatures1,
       author = {{Meerburg}, P. Daniel and {Spergel}, David N. and {Wandelt}, Benjamin D.},
        title = "{Searching for oscillations in the primordial power spectrum. II. Constraints from Planck data}",
      journal = {\prd},
     keywords = {98.80.Es, Observational cosmology, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2014,
        month = mar,
       volume = {89},
       number = {6},
          eid = {063537},
        pages = {063537},
          doi = {10.1103/PhysRevD.89.063537},
archivePrefix = {arXiv},
       eprint = {1308.3705},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014PhRvD..89f3537M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{SearchingFeatures2,
       author = {{Chen}, Xingang and {Namjoo}, Mohammad Hossein and {Wang}, Yi},
        title = "{Models of the Primordial Standard Clock}",
      journal = {\jcap},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, High Energy Physics - Phenomenology, High Energy Physics - Theory},
         year = 2015,
        month = feb,
       volume = {2015},
       number = {2},
        pages = {027-027},
          doi = {10.1088/1475-7516/2015/02/027},
archivePrefix = {arXiv},
       eprint = {1411.2349},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015JCAP...02..027C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{PlanckInflation13,
       author = {{Planck Collaboration} and {Ade}, P.~A.~R. and {Aghanim}, N. and {Armitage-Caplan}, C. and {Arnaud}, M. and {Ashdown}, M. and {Atrio-Barandela}, F. and {Aumont}, J. and {Baccigalupi}, C. and {Banday}, A.~J. and {Barreiro}, R.~B. and {Bartlett}, J.~G. and {Bartolo}, N. and {Battaner}, E. and {Benabed}, K. and {Beno{\^\i}t}, A. and {Benoit-L{\'e}vy}, A. and {Bernard}, J. -P. and {Bersanelli}, M. and {Bielewicz}, P. and {Bobin}, J. and {Bock}, J.~J. and {Bonaldi}, A. and {Bond}, J.~R. and {Borrill}, J. and {Bouchet}, F.~R. and {Bridges}, M. and {Bucher}, M. and {Burigana}, C. and {Butler}, R.~C. and {Calabrese}, E. and {Cardoso}, J. -F. and {Catalano}, A. and {Challinor}, A. and {Chamballu}, A. and {Chiang}, H.~C. and {Chiang}, L. -Y. and {Christensen}, P.~R. and {Church}, S. and {Clements}, D.~L. and {Colombi}, S. and {Colombo}, L.~P.~L. and {Couchot}, F. and {Coulais}, A. and {Crill}, B.~P. and {Curto}, A. and {Cuttaia}, F. and {Danese}, L. and {Davies}, R.~D. and {Davis}, R.~J. and {de Bernardis}, P. and {de Rosa}, A. and {de Zotti}, G. and {Delabrouille}, J. and {Delouis}, J. -M. and {D{\'e}sert}, F. -X. and {Dickinson}, C. and {Diego}, J.~M. and {Dole}, H. and {Donzelli}, S. and {Dor{\'e}}, O. and {Douspis}, M. and {Dunkley}, J. and {Dupac}, X. and {Efstathiou}, G. and {En{\ss}lin}, T.~A. and {Eriksen}, H.~K. and {Finelli}, F. and {Forni}, O. and {Frailis}, M. and {Franceschi}, E. and {Galeotta}, S. and {Ganga}, K. and {Gauthier}, C. and {Giard}, M. and {Giardino}, G. and {Giraud-H{\'e}raud}, Y. and {Gonz{\'a}lez-Nuevo}, J. and {G{\'o}rski}, K.~M. and {Gratton}, S. and {Gregorio}, A. and {Gruppuso}, A. and {Hamann}, J. and {Hansen}, F.~K. and {Hanson}, D. and {Harrison}, D. and {Henrot-Versill{\'e}}, S. and {Hern{\'a}ndez-Monteagudo}, C. and {Herranz}, D. and {Hildebrandt}, S.~R. and {Hivon}, E. and {Hobson}, M. and {Holmes}, W.~A. and {Hornstrup}, A. and {Hovest}, W. and {Huffenberger}, K.~M. and {Jaffe}, A.~H. and {Jaffe}, T.~R. and {Jones}, W.~C. and {Juvela}, M. and {Keih{\"a}nen}, E. and {Keskitalo}, R. and {Kisner}, T.~S. and {Kneissl}, R. and {Knoche}, J. and {Knox}, L. and {Kunz}, M. and {Kurki-Suonio}, H. and {Lagache}, G. and {L{\"a}hteenm{\"a}ki}, A. and {Lamarre}, J. -M. and {Lasenby}, A. and {Laureijs}, R.~J. and {Lawrence}, C.~R. and {Leach}, S. and {Leahy}, J.~P. and {Leonardi}, R. and {Lesgourgues}, J. and {Lewis}, A. and {Liguori}, M. and {Lilje}, P.~B. and {Linden-V{\o}rnle}, M. and {L{\'o}pez-Caniego}, M. and {Lubin}, P.~M. and {Mac{\'\i}as-P{\'e}rez}, J.~F. and {Maffei}, B. and {Maino}, D. and {Mandolesi}, N. and {Maris}, M. and {Marshall}, D.~J. and {Martin}, P.~G. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Masi}, S. and {Massardi}, M. and {Matarrese}, S. and {Matthai}, F. and {Mazzotta}, P. and {Meinhold}, P.~R. and {Melchiorri}, A. and {Mendes}, L. and {Mennella}, A. and {Migliaccio}, M. and {Mitra}, S. and {Miville-Desch{\^e}nes}, M. -A. and {Moneti}, A. and {Montier}, L. and {Morgante}, G. and {Mortlock}, D. and {Moss}, A. and {Munshi}, D. and {Murphy}, J.~A. and {Naselsky}, P. and {Nati}, F. and {Natoli}, P. and {Netterfield}, C.~B. and {N{\o}rgaard-Nielsen}, H.~U. and {Noviello}, F. and {Novikov}, D. and {Novikov}, I. and {O'Dwyer}, I.~J. and {Osborne}, S. and {Oxborrow}, C.~A. and {Paci}, F. and {Pagano}, L. and {Pajot}, F. and {Paladini}, R. and {Pandolfi}, S. and {Paoletti}, D. and {Partridge}, B. and {Pasian}, F. and {Patanchon}, G. and {Peiris}, H.~V. and {Perdereau}, O. and {Perotto}, L. and {Perrotta}, F. and {Piacentini}, F. and {Piat}, M. and {Pierpaoli}, E. and {Pietrobon}, D. and {Plaszczynski}, S. and {Pointecouteau}, E. and {Polenta}, G. and {Ponthieu}, N. and {Popa}, L. and {Poutanen}, T. and {Pratt}, G.~W. and {Pr{\'e}zeau}, G. and {Prunet}, S. and {Puget}, J. -L. and {Rachen}, J.~P. and {Rebolo}, R. and {Reinecke}, M. and {Remazeilles}, M. and {Renault}, C. and {Ricciardi}, S. and {Riller}, T. and {Ristorcelli}, I. and {Rocha}, G. and {Rosset}, C. and {Roudier}, G. and {Rowan-Robinson}, M. and {Rubi{\~n}o-Mart{\'\i}n}, J.~A. and {Rusholme}, B. and {Sandri}, M. and {Santos}, D. and {Savelainen}, M. and {Savini}, G. and {Scott}, D. and {Seiffert}, M.~D. and {Shellard}, E.~P.~S. and {Spencer}, L.~D. and {Starck}, J. -L. and {Stolyarov}, V. and {Stompor}, R. and {Sudiwala}, R. and {Sunyaev}, R. and {Sureau}, F. and {Sutton}, D. and {Suur-Uski}, A. -S. and {Sygnet}, J. -F. and {Tauber}, J.~A. and {Tavagnacco}, D. and {Terenzi}, L. and {Toffolatti}, L. and {Tomasi}, M. and {Tr{\'e}guer-Goudineau}, J. and {Tristram}, M. and {Tucci}, M. and {Tuovinen}, J. and {Valenziano}, L. and {Valiviita}, J. and {Van Tent}, B. and {Varis}, J. and {Vielva}, P. and {Villa}, F. and {Vittorio}, N. and {Wade}, L.~A. and {Wandelt}, B.~D. and {White}, M. and {Wilkinson}, A. and {Yvon}, D. and {Zacchei}, A. and {Zibin}, J.~P. and {Zonca}, A.},
        title = "{Planck 2013 results. XXII. Constraints on inflation}",
      journal = {\aap},
     keywords = {cosmic background radiation, inflation, early Universe, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2014,
        month = nov,
       volume = {571},
          eid = {A22},
        pages = {A22},
          doi = {10.1051/0004-6361/201321569},
archivePrefix = {arXiv},
       eprint = {1303.5082},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014A&A...571A..22P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ReconOldReconstructions,
       author = {{V{\'a}zquez}, J. Alberto and {Bridges}, M. and {Hobson}, M.~P. and {Lasenby}, A.~N.},
        title = "{Model selection applied to reconstruction of the Primordial Power Spectrum}",
      journal = {\jcap},
     keywords = {Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2012,
        month = jun,
       volume = {2012},
       number = {6},
          eid = {006},
        pages = {006},
          doi = {10.1088/1475-7516/2012/06/006},
archivePrefix = {arXiv},
       eprint = {1203.1252},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012JCAP...06..006V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{WillPaper13,
       author = {{Aslanyan}, Grigor and {Price}, Layne C. and {Abazajian}, Kevork N. and {Easther}, Richard},
        title = "{The Knotted Sky I: Planck constraints on the primordial power spectrum}",
      journal = {\jcap},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, High Energy Physics - Phenomenology},
         year = 2014,
        month = aug,
       volume = {2014},
       number = {8},
        pages = {052-052},
          doi = {10.1088/1475-7516/2014/08/052},
archivePrefix = {arXiv},
       eprint = {1403.5849},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014JCAP...08..052A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ReconCMBlike,
       author = {{Gauthier}, Christopher and {Bucher}, Martin},
        title = "{Reconstructing the primordial power spectrum from the CMB}",
      journal = {\jcap},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2012,
        month = oct,
       volume = {2012},
       number = {10},
          eid = {050},
        pages = {050},
          doi = {10.1088/1475-7516/2012/10/050},
archivePrefix = {arXiv},
       eprint = {1209.2147},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012JCAP...10..050G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Planck18Parameters,
       author = {{Planck Collaboration} and {Aghanim}, N. and {Akrami}, Y. and {Ashdown}, M. and {Aumont}, J. and {Baccigalupi}, C. and {Ballardini}, M. and {Banday}, A.~J. and {Barreiro}, R.~B. and {Bartolo}, N. and {Basak}, S. and {Battye}, R. and {Benabed}, K. and {Bernard}, J. -P. and {Bersanelli}, M. and {Bielewicz}, P. and {Bock}, J.~J. and {Bond}, J.~R. and {Borrill}, J. and {Bouchet}, F.~R. and {Boulanger}, F. and {Bucher}, M. and {Burigana}, C. and {Butler}, R.~C. and {Calabrese}, E. and {Cardoso}, J. -F. and {Carron}, J. and {Challinor}, A. and {Chiang}, H.~C. and {Chluba}, J. and {Colombo}, L.~P.~L. and {Combet}, C. and {Contreras}, D. and {Crill}, B.~P. and {Cuttaia}, F. and {de Bernardis}, P. and {de Zotti}, G. and {Delabrouille}, J. and {Delouis}, J. -M. and {Di Valentino}, E. and {Diego}, J.~M. and {Dor{\'e}}, O. and {Douspis}, M. and {Ducout}, A. and {Dupac}, X. and {Dusini}, S. and {Efstathiou}, G. and {Elsner}, F. and {En{\ss}lin}, T.~A. and {Eriksen}, H.~K. and {Fantaye}, Y. and {Farhang}, M. and {Fergusson}, J. and {Fernandez-Cobos}, R. and {Finelli}, F. and {Forastieri}, F. and {Frailis}, M. and {Fraisse}, A.~A. and {Franceschi}, E. and {Frolov}, A. and {Galeotta}, S. and {Galli}, S. and {Ganga}, K. and {G{\'e}nova-Santos}, R.~T. and {Gerbino}, M. and {Ghosh}, T. and {Gonz{\'a}lez-Nuevo}, J. and {G{\'o}rski}, K.~M. and {Gratton}, S. and {Gruppuso}, A. and {Gudmundsson}, J.~E. and {Hamann}, J. and {Handley}, W. and {Hansen}, F.~K. and {Herranz}, D. and {Hildebrandt}, S.~R. and {Hivon}, E. and {Huang}, Z. and {Jaffe}, A.~H. and {Jones}, W.~C. and {Karakci}, A. and {Keih{\"a}nen}, E. and {Keskitalo}, R. and {Kiiveri}, K. and {Kim}, J. and {Kisner}, T.~S. and {Knox}, L. and {Krachmalnicoff}, N. and {Kunz}, M. and {Kurki-Suonio}, H. and {Lagache}, G. and {Lamarre}, J. -M. and {Lasenby}, A. and {Lattanzi}, M. and {Lawrence}, C.~R. and {Le Jeune}, M. and {Lemos}, P. and {Lesgourgues}, J. and {Levrier}, F. and {Lewis}, A. and {Liguori}, M. and {Lilje}, P.~B. and {Lilley}, M. and {Lindholm}, V. and {L{\'o}pez-Caniego}, M. and {Lubin}, P.~M. and {Ma}, Y. -Z. and {Mac{\'\i}as-P{\'e}rez}, J.~F. and {Maggio}, G. and {Maino}, D. and {Mandolesi}, N. and {Mangilli}, A. and {Marcos-Caballero}, A. and {Maris}, M. and {Martin}, P.~G. and {Martinelli}, M. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Matarrese}, S. and {Mauri}, N. and {McEwen}, J.~D. and {Meinhold}, P.~R. and {Melchiorri}, A. and {Mennella}, A. and {Migliaccio}, M. and {Millea}, M. and {Mitra}, S. and {Miville-Desch{\^e}nes}, M. -A. and {Molinari}, D. and {Montier}, L. and {Morgante}, G. and {Moss}, A. and {Natoli}, P. and {N{\o}rgaard-Nielsen}, H.~U. and {Pagano}, L. and {Paoletti}, D. and {Partridge}, B. and {Patanchon}, G. and {Peiris}, H.~V. and {Perrotta}, F. and {Pettorino}, V. and {Piacentini}, F. and {Polastri}, L. and {Polenta}, G. and {Puget}, J. -L. and {Rachen}, J.~P. and {Reinecke}, M. and {Remazeilles}, M. and {Renzi}, A. and {Rocha}, G. and {Rosset}, C. and {Roudier}, G. and {Rubi{\~n}o-Mart{\'\i}n}, J.~A. and {Ruiz-Granados}, B. and {Salvati}, L. and {Sandri}, M. and {Savelainen}, M. and {Scott}, D. and {Shellard}, E.~P.~S. and {Sirignano}, C. and {Sirri}, G. and {Spencer}, L.~D. and {Sunyaev}, R. and {Suur-Uski}, A. -S. and {Tauber}, J.~A. and {Tavagnacco}, D. and {Tenti}, M. and {Toffolatti}, L. and {Tomasi}, M. and {Trombetti}, T. and {Valenziano}, L. and {Valiviita}, J. and {Van Tent}, B. and {Vibert}, L. and {Vielva}, P. and {Villa}, F. and {Vittorio}, N. and {Wandelt}, B.~D. and {Wehus}, I.~K. and {White}, M. and {White}, S.~D.~M. and {Zacchei}, A. and {Zonca}, A.},
        title = "{Planck 2018 results. VI. Cosmological parameters}",
      journal = {\aap},
     keywords = {cosmic background radiation, cosmological parameters, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = sep,
       volume = {641},
          eid = {A6},
        pages = {A6},
          doi = {10.1051/0004-6361/201833910},
archivePrefix = {arXiv},
       eprint = {1807.06209},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...641A...6P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{InflaBrout1978,
title = {The creation of the universe as a quantum phenomenon},
journal = {Annals of Physics},
volume = {115},
number = {1},
pages = {78-106},
year = {1978},
issn = {0003-4916},
doi = {https://doi.org/10.1016/0003-4916(78)90176-8},
url = {https://www.sciencedirect.com/science/article/pii/0003491678901768},
author = {R Brout and F Englert and E Gunzig},
abstract = {Quantum creation of massy particles can occur in the cosmological context without cost of energy. This fact is seized upon to construct a causal open homogeneous isotropic cosmology. The universe is conceived as the response of matter and the gravitational field to a spontaneous pointlike disturbance. Its history unfolds in two stages, creation and free expansion. The first stage gives rise to a “fireball.” The free expansion is extrapolated back to the “fireball.” The latter thus replaces the “big-bang,” thereby avoiding an initial singularity. Though not intrinsic to the theory it does suggest the interpretation of the cosmological part of the gravitational field as the scalar dilaton that is encountered in the dynamical generation of mass in conformally invariant theory.}
}

@article{InflaStarobinski1980,
title = {A new type of isotropic cosmological models without singularity},
journal = {Physics Letters B},
volume = {91},
number = {1},
pages = {99-102},
year = {1980},
issn = {0370-2693},
doi = {https://doi.org/10.1016/0370-2693(80)90670-X},
url = {https://www.sciencedirect.com/science/article/pii/037026938090670X},
author = {A.A. Starobinsky},
abstract = {The Einstein equations with quantum one-loop contributions of conformally covariant matter fields are shown to admit a class of nonsingular isotropic homogeneous solutions that correspond to a picture of the Universe being initially in the most symmetric (de Sitter) state.}
}

@article{InflaGuth1981,
  title = {Inflationary universe: A possible solution to the horizon and flatness problems},
  author = {Guth, Alan H.},
  journal = {Phys. Rev. D},
  volume = {23},
  issue = {2},
  pages = {347--356},
  numpages = {0},
  year = {1981},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.23.347},
  url = {https://link.aps.org/doi/10.1103/PhysRevD.23.347}
}

@article{InflaLinde1982,
title = {A new inflationary universe scenario: A possible solution of the horizon, flatness, homogeneity, isotropy and primordial monopole problems},
journal = {Physics Letters B},
volume = {108},
number = {6},
pages = {389-393},
year = {1982},
issn = {0370-2693},
doi = {https://doi.org/10.1016/0370-2693(82)91219-9},
url = {https://www.sciencedirect.com/science/article/pii/0370269382912199},
author = {A.D. Linde},
abstract = {A new inflationary universe scenario is suggested, which is free of the shortcomings of the previous one and provides a possible solution of the horizon, flatness, homogeneity and isotropy problems in cosmology, and also a solution of the primordial monopole problem in grand unified theories.}
}

@article{InflaAlbrechtSteinhardt1982,
  title = {Cosmology for Grand Unified Theories with Radiatively Induced Symmetry Breaking},
  author = {Albrecht, Andreas and Steinhardt, Paul J.},
  journal = {Phys. Rev. Lett.},
  volume = {48},
  issue = {17},
  pages = {1220--1223},
  numpages = {0},
  year = {1982},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.48.1220},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.48.1220}
}

@article{InflaLinde1983,
title = {Chaotic inflation},
journal = {Physics Letters B},
volume = {129},
number = {3},
pages = {177-181},
year = {1983},
issn = {0370-2693},
doi = {https://doi.org/10.1016/0370-2693(83)90837-7},
url = {https://www.sciencedirect.com/science/article/pii/0370269383908377},
author = {A.D. Linde},
abstract = {A new scenario of the very early stages of the evolution of the universe is suggested. According to this scenario, inflation is a natural (and may be even inevitable) consequence of chaotic initial conditions in the early universe.}
}

@ARTICLE{AnomaliesSupression,
       author = {{Copi}, Craig J. and {Huterer}, Dragan and {Schwarz}, Dominik J. and {Starkman}, Glenn D.},
        title = "{Lack of large-angle TT correlations persists in WMAP and Planck}",
      journal = {\mnras},
     keywords = {cosmic background radiation, large-scale structure of Universe, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2015,
        month = aug,
       volume = {451},
       number = {3},
        pages = {2978-2985},
          doi = {10.1093/mnras/stv1143},
archivePrefix = {arXiv},
       eprint = {1310.3831},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.451.2978C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ModelAdams2001,
       author = {{Adams}, Jennifer and {Cresswell}, Bevan and {Easther}, Richard},
        title = "{Inflationary perturbations from a potential with a step}",
      journal = {\prd},
     keywords = {98.80.Cq, Particle-theory and field-theory models of the early Universe, Astrophysics},
         year = 2001,
        month = dec,
       volume = {64},
       number = {12},
        pages = {123514},
          doi = {10.1103/PhysRevD.64.123514},
archivePrefix = {arXiv},
       eprint = {astro-ph/0102236},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001PhRvD..64l3514A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{ModelAchucarro2010,
       author = {{Ach{\'u}carro}, Ana and {Gong}, Jinn-Ouk and {Hardeman}, Sjoerd and {Palma}, Gonzalo A. and {Patil}, Subodh P.},
        title = "{Features of heavy physics in the CMB power spectrum}",
      journal = {\jcap},
     keywords = {High Energy Physics - Phenomenology, Astrophysics - Cosmology and Nongalactic Astrophysics, General Relativity and Quantum Cosmology, High Energy Physics - Theory},
         year = 2011,
        month = jan,
       volume = {2011},
       number = {1},
          eid = {030},
        pages = {030},
          doi = {10.1088/1475-7516/2011/01/030},
archivePrefix = {arXiv},
       eprint = {1010.3693},
 primaryClass = {hep-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011JCAP...01..030A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ModelMartin2001,
       author = {{Martin}, J{\'e}r{\^o}me and {Brandenberger}, Robert H.},
        title = "{Trans-Planckian problem of inflationary cosmology}",
      journal = {\prd},
     keywords = {98.80.Cq, 98.70.Vc, Particle-theory and field-theory models of the early Universe, Background radiations, High Energy Physics - Theory, Astrophysics, General Relativity and Quantum Cosmology, High Energy Physics - Phenomenology},
         year = 2001,
        month = jun,
       volume = {63},
       number = {12},
          eid = {123501},
        pages = {123501},
          doi = {10.1103/PhysRevD.63.123501},
archivePrefix = {arXiv},
       eprint = {hep-th/0005209},
 primaryClass = {hep-th},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001PhRvD..63l3501M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{ModelMartin2003,
       author = {{Martin}, J{\'e}r{\^o}me and {Brandenberger}, Robert},
        title = "{Dependence of the spectra of fluctuations in inflationary cosmology on trans-Planckian physics}",
      journal = {\prd},
     keywords = {98.80.Cq, 98.70.Vc, Particle-theory and field-theory models of the early Universe, Background radiations, High Energy Physics - Theory, Astrophysics, General Relativity and Quantum Cosmology, High Energy Physics - Phenomenology},
         year = 2003,
        month = sep,
       volume = {68},
       number = {6},
          eid = {063513},
        pages = {063513},
          doi = {10.1103/PhysRevD.68.063513},
archivePrefix = {arXiv},
       eprint = {hep-th/0305161},
 primaryClass = {hep-th},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003PhRvD..68f3513M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{ModelBozza2003,
       author = {{Bozza}, V. and {Giovannini}, M. and {Veneziano}, G.},
        title = "{Cosmological perturbations from a new-physics hypersurface}",
      journal = {\jcap},
     keywords = {High Energy Physics - Theory, General Relativity and Quantum Cosmology, High Energy Physics - Phenomenology},
         year = 2003,
        month = may,
       volume = {2003},
       number = {5},
          eid = {001},
        pages = {001},
          doi = {10.1088/1475-7516/2003/05/001},
archivePrefix = {arXiv},
       eprint = {hep-th/0302184},
 primaryClass = {hep-th},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003JCAP...05..001B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ModelFlauger2017,
       author = {{Flauger}, Raphael and {McAllister}, Liam and {Silverstein}, Eva and {Westphal}, Alexander},
        title = "{Drifting oscillations in axion monodromy}",
      journal = {\jcap},
     keywords = {High Energy Physics - Theory, Astrophysics - Cosmology and Nongalactic Astrophysics, High Energy Physics - Phenomenology},
         year = 2017,
        month = oct,
       volume = {2017},
       number = {10},
          eid = {055},
        pages = {055},
          doi = {10.1088/1475-7516/2017/10/055},
archivePrefix = {arXiv},
       eprint = {1412.1814},
 primaryClass = {hep-th},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017JCAP...10..055F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ModelLinearOsci,
       author = {{Meerburg}, P. Daniel and {Spergel}, David N. and {Wandelt}, Benjamin D.},
        title = "{Searching for oscillations in the primordial power spectrum. II. Constraints from Planck data}",
      journal = {\prd},
     keywords = {98.80.Es, Observational cosmology, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2014,
        month = mar,
       volume = {89},
       number = {6},
          eid = {063537},
        pages = {063537},
          doi = {10.1103/PhysRevD.89.063537},
archivePrefix = {arXiv},
       eprint = {1308.3705},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014PhRvD..89f3537M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ModelJackson2013,
       author = {{Jackson}, Mark G. and {Shiu}, Gary},
        title = "{Study of the consistency relation for single-field inflation with power spectrum oscillations}",
      journal = {\prd},
     keywords = {98.80.Cq, 98.80.Es, Particle-theory and field-theory models of the early Universe, Observational cosmology, High Energy Physics - Theory, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2013,
        month = dec,
       volume = {88},
       number = {12},
          eid = {123511},
        pages = {123511},
          doi = {10.1103/PhysRevD.88.123511},
archivePrefix = {arXiv},
       eprint = {1303.4973},
 primaryClass = {hep-th},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013PhRvD..88l3511J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ModelDanielsson2002,
       author = {{Danielsson}, Ulf H.},
        title = "{Note on inflation and trans-Planckian physics}",
      journal = {\prd},
     keywords = {98.80.Cq, Particle-theory and field-theory models of the early Universe, High Energy Physics - Theory, Astrophysics},
         year = 2002,
        month = jul,
       volume = {66},
       number = {2},
          eid = {023511},
        pages = {023511},
          doi = {10.1103/PhysRevD.66.023511},
archivePrefix = {arXiv},
       eprint = {hep-th/0203198},
 primaryClass = {hep-th},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002PhRvD..66b3511D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ModelChen2012,
       author = {{Chen}, Xingang},
        title = "{Primordial Features as Evidence for Inflation}",
      journal = {arXiv e-prints},
     keywords = {High Energy Physics - Theory, Astrophysics - Cosmology and Extragalactic Astrophysics, High Energy Physics - Phenomenology},
         year = 2011,
        month = apr,
          eid = {arXiv:1104.1323},
        pages = {arXiv:1104.1323},
archivePrefix = {arXiv},
       eprint = {1104.1323},
 primaryClass = {hep-th},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011arXiv1104.1323C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ModelContaldi2003,
       author = {{Contaldi}, Carlo R. and {Peloso}, Marco and {Kofman}, Lev and {Linde}, Andrei},
        title = "{Suppressing the lower multipoles in the CMB anisotropies}",
      journal = {\jcap},
     keywords = {Astrophysics, General Relativity and Quantum Cosmology, High Energy Physics - Phenomenology, High Energy Physics - Theory},
         year = 2003,
        month = jul,
       volume = {2003},
       number = {7},
          eid = {002},
        pages = {002},
          doi = {10.1088/1475-7516/2003/07/002},
archivePrefix = {arXiv},
       eprint = {astro-ph/0303636},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003JCAP...07..002C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ModeSinha2006,
       author = {{Sinha}, Rita and {Souradeep}, Tarun},
        title = "{Post-WMAP assessment of infrared cutoff in the primordial spectrum from inflation}",
      journal = {\prd},
     keywords = {98.80.Cq, 98.80.-k, Particle-theory and field-theory models of the early Universe, Cosmology, Astrophysics},
         year = 2006,
        month = aug,
       volume = {74},
       number = {4},
          eid = {043518},
        pages = {043518},
          doi = {10.1103/PhysRevD.74.043518},
archivePrefix = {arXiv},
       eprint = {astro-ph/0511808},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006PhRvD..74d3518S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{AnomaliesHemispherical1,
       author = {{Schwarz}, Dominik J. and {Copi}, Craig J. and {Huterer}, Dragan and {Starkman}, Glenn D.},
        title = "{CMB anomalies after Planck}",
      journal = {Classical and Quantum Gravity},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2016,
        month = sep,
       volume = {33},
       number = {18},
          eid = {184001},
        pages = {184001},
          doi = {10.1088/0264-9381/33/18/184001},
archivePrefix = {arXiv},
       eprint = {1510.07929},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016CQGra..33r4001S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{AnomaliesHemisphericalWMAP7,
       author = {{Paci}, F. and {Gruppuso}, A. and {Finelli}, F. and {De Rosa}, A. and {Mandolesi}, N. and {Natoli}, P.},
        title = "{Hemispherical power asymmetries in the WMAP 7-year low-resolution temperature and polarization maps}",
      journal = {\mnras},
     keywords = {methods: data analysis, methods: statistical, cosmic background radiation, cosmology: observations, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = oct,
       volume = {434},
       number = {4},
        pages = {3071-3077},
          doi = {10.1093/mnras/stt1219},
archivePrefix = {arXiv},
       eprint = {1301.5195},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.434.3071P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{AnomaliesOddParity,
       author = {{Akrami}, Y. and {Fantaye}, Y. and {Shafieloo}, A. and {Eriksen}, H.~K. and {Hansen}, F.~K. and {Banday}, A.~J. and {G{\'o}rski}, K.~M.},
        title = "{Power Asymmetry in WMAP and Planck Temperature Sky Maps as Measured by a Local Variance Estimator}",
      journal = {\apjl},
     keywords = {cosmic background radiation, cosmology: observations, methods: statistical, Astrophysics - Cosmology and Nongalactic Astrophysics, Physics - Data Analysis, Statistics and Probability},
         year = 2014,
        month = apr,
       volume = {784},
       number = {2},
          eid = {L42},
        pages = {L42},
          doi = {10.1088/2041-8205/784/2/L42},
archivePrefix = {arXiv},
       eprint = {1402.0870},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...784L..42A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{AnomaliesPlanck18,
       author = {{Planck Collaboration} and {Akrami}, Y. and {Ashdown}, M. and {Aumont}, J. and {Baccigalupi}, C. and {Ballardini}, M. and {Banday}, A.~J. and {Barreiro}, R.~B. and {Bartolo}, N. and {Basak}, S. and {Benabed}, K. and {Bersanelli}, M. and {Bielewicz}, P. and {Bock}, J.~J. and {Bond}, J.~R. and {Borrill}, J. and {Bouchet}, F.~R. and {Boulanger}, F. and {Bucher}, M. and {Burigana}, C. and {Butler}, R.~C. and {Calabrese}, E. and {Cardoso}, J. -F. and {Casaponsa}, B. and {Chiang}, H.~C. and {Colombo}, L.~P.~L. and {Combet}, C. and {Contreras}, D. and {Crill}, B.~P. and {de Bernardis}, P. and {de Zotti}, G. and {Delabrouille}, J. and {Delouis}, J. -M. and {Di Valentino}, E. and {Diego}, J.~M. and {Dor{\'e}}, O. and {Douspis}, M. and {Ducout}, A. and {Dupac}, X. and {Efstathiou}, G. and {Elsner}, F. and {En{\ss}lin}, T.~A. and {Eriksen}, H.~K. and {Fantaye}, Y. and {Fernandez-Cobos}, R. and {Finelli}, F. and {Frailis}, M. and {Fraisse}, A.~A. and {Franceschi}, E. and {Frolov}, A. and {Galeotta}, S. and {Galli}, S. and {Ganga}, K. and {G{\'e}nova-Santos}, R.~T. and {Gerbino}, M. and {Ghosh}, T. and {Gonz{\'a}lez-Nuevo}, J. and {G{\'o}rski}, K.~M. and {Gruppuso}, A. and {Gudmundsson}, J.~E. and {Hamann}, J. and {Handley}, W. and {Hansen}, F.~K. and {Herranz}, D. and {Hivon}, E. and {Huang}, Z. and {Jaffe}, A.~H. and {Jones}, W.~C. and {Keih{\"a}nen}, E. and {Keskitalo}, R. and {Kiiveri}, K. and {Kim}, J. and {Krachmalnicoff}, N. and {Kunz}, M. and {Kurki-Suonio}, H. and {Lagache}, G. and {Lamarre}, J. -M. and {Lasenby}, A. and {Lattanzi}, M. and {Lawrence}, C.~R. and {Le Jeune}, M. and {Levrier}, F. and {Liguori}, M. and {Lilje}, P.~B. and {Lindholm}, V. and {L{\'o}pez-Caniego}, M. and {Ma}, Y. -Z. and {Mac{\'\i}as-P{\'e}rez}, J.~F. and {Maggio}, G. and {Maino}, D. and {Mandolesi}, N. and {Mangilli}, A. and {Marcos-Caballero}, A. and {Maris}, M. and {Martin}, P.~G. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Matarrese}, S. and {Mauri}, N. and {McEwen}, J.~D. and {Meinhold}, P.~R. and {Mennella}, A. and {Migliaccio}, M. and {Miville-Desch{\^e}nes}, M. -A. and {Molinari}, D. and {Moneti}, A. and {Montier}, L. and {Morgante}, G. and {Moss}, A. and {Natoli}, P. and {Pagano}, L. and {Paoletti}, D. and {Partridge}, B. and {Perrotta}, F. and {Pettorino}, V. and {Piacentini}, F. and {Polenta}, G. and {Puget}, J. -L. and {Rachen}, J.~P. and {Reinecke}, M. and {Remazeilles}, M. and {Renzi}, A. and {Rocha}, G. and {Rosset}, C. and {Roudier}, G. and {Rubi{\~n}o-Mart{\'\i}n}, J.~A. and {Ruiz-Granados}, B. and {Salvati}, L. and {Savelainen}, M. and {Scott}, D. and {Shellard}, E.~P.~S. and {Sirignano}, C. and {Sunyaev}, R. and {Suur-Uski}, A. -S. and {Tauber}, J.~A. and {Tavagnacco}, D. and {Tenti}, M. and {Toffolatti}, L. and {Tomasi}, M. and {Trombetti}, T. and {Valenziano}, L. and {Valiviita}, J. and {Van Tent}, B. and {Vielva}, P. and {Villa}, F. and {Vittorio}, N. and {Wandelt}, B.~D. and {Wehus}, I.~K. and {Zacchei}, A. and {Zibin}, J.~P. and {Zonca}, A.},
        title = "{Planck 2018 results. VII. Isotropy and statistics of the CMB}",
      journal = {\aap},
     keywords = {cosmology: observations, cosmic background radiation, polarization, methods: data analysis, methods: statistical, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = sep,
       volume = {641},
          eid = {A7},
        pages = {A7},
          doi = {10.1051/0004-6361/201935201},
archivePrefix = {arXiv},
       eprint = {1906.02552},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...641A...7P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{AnomaliesColdSpot1,
    author = "Cruz, M. and Martinez-Gonzalez, E. and Vielva, P.",
    editor = "Diego, Jose M. and Goicoechea, Luis J. and Gonzalez-Serrano, J. Ignacio and Gorgas, Javier",
    title = "{The WMAP cold spot}",
    eprint = "0901.1986",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1007/978-3-642-11250-8_37",
    journal = "Astrophys. Space Sci. Proc.",
    pages = "275",
    year = "2010"
}

@ARTICLE{AnomaliesColdSpot2,
       author = {{Vielva}, Patricio},
        title = "{A Comprehensive Overview of the Cold Spot}",
      journal = {Advances in Astronomy},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2010,
        month = jan,
       volume = {2010},
          eid = {592094},
        pages = {592094},
          doi = {10.1155/2010/592094},
archivePrefix = {arXiv},
       eprint = {1008.3051},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010AdAst2010E..77V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Planck15Parameters,
       author = {{Planck Collaboration} and {Ade}, P.~A.~R. and {Aghanim}, N. and {Arnaud}, M. and {Ashdown}, M. and {Aumont}, J. and {Baccigalupi}, C. and {Banday}, A.~J. and {Barreiro}, R.~B. and {Bartlett}, J.~G. and {Bartolo}, N. and {Battaner}, E. and {Battye}, R. and {Benabed}, K. and {Beno{\^\i}t}, A. and {Benoit-L{\'e}vy}, A. and {Bernard}, J. -P. and {Bersanelli}, M. and {Bielewicz}, P. and {Bock}, J.~J. and {Bonaldi}, A. and {Bonavera}, L. and {Bond}, J.~R. and {Borrill}, J. and {Bouchet}, F.~R. and {Boulanger}, F. and {Bucher}, M. and {Burigana}, C. and {Butler}, R.~C. and {Calabrese}, E. and {Cardoso}, J. -F. and {Catalano}, A. and {Challinor}, A. and {Chamballu}, A. and {Chary}, R. -R. and {Chiang}, H.~C. and {Chluba}, J. and {Christensen}, P.~R. and {Church}, S. and {Clements}, D.~L. and {Colombi}, S. and {Colombo}, L.~P.~L. and {Combet}, C. and {Coulais}, A. and {Crill}, B.~P. and {Curto}, A. and {Cuttaia}, F. and {Danese}, L. and {Davies}, R.~D. and {Davis}, R.~J. and {de Bernardis}, P. and {de Rosa}, A. and {de Zotti}, G. and {Delabrouille}, J. and {D{\'e}sert}, F. -X. and {Di Valentino}, E. and {Dickinson}, C. and {Diego}, J.~M. and {Dolag}, K. and {Dole}, H. and {Donzelli}, S. and {Dor{\'e}}, O. and {Douspis}, M. and {Ducout}, A. and {Dunkley}, J. and {Dupac}, X. and {Efstathiou}, G. and {Elsner}, F. and {En{\ss}lin}, T.~A. and {Eriksen}, H.~K. and {Farhang}, M. and {Fergusson}, J. and {Finelli}, F. and {Forni}, O. and {Frailis}, M. and {Fraisse}, A.~A. and {Franceschi}, E. and {Frejsel}, A. and {Galeotta}, S. and {Galli}, S. and {Ganga}, K. and {Gauthier}, C. and {Gerbino}, M. and {Ghosh}, T. and {Giard}, M. and {Giraud-H{\'e}raud}, Y. and {Giusarma}, E. and {Gjerl{\o}w}, E. and {Gonz{\'a}lez-Nuevo}, J. and {G{\'o}rski}, K.~M. and {Gratton}, S. and {Gregorio}, A. and {Gruppuso}, A. and {Gudmundsson}, J.~E. and {Hamann}, J. and {Hansen}, F.~K. and {Hanson}, D. and {Harrison}, D.~L. and {Helou}, G. and {Henrot-Versill{\'e}}, S. and {Hern{\'a}ndez-Monteagudo}, C. and {Herranz}, D. and {Hildebrandt}, S.~R. and {Hivon}, E. and {Hobson}, M. and {Holmes}, W.~A. and {Hornstrup}, A. and {Hovest}, W. and {Huang}, Z. and {Huffenberger}, K.~M. and {Hurier}, G. and {Jaffe}, A.~H. and {Jaffe}, T.~R. and {Jones}, W.~C. and {Juvela}, M. and {Keih{\"a}nen}, E. and {Keskitalo}, R. and {Kisner}, T.~S. and {Kneissl}, R. and {Knoche}, J. and {Knox}, L. and {Kunz}, M. and {Kurki-Suonio}, H. and {Lagache}, G. and {L{\"a}hteenm{\"a}ki}, A. and {Lamarre}, J. -M. and {Lasenby}, A. and {Lattanzi}, M. and {Lawrence}, C.~R. and {Leahy}, J.~P. and {Leonardi}, R. and {Lesgourgues}, J. and {Levrier}, F. and {Lewis}, A. and {Liguori}, M. and {Lilje}, P.~B. and {Linden-V{\o}rnle}, M. and {L{\'o}pez-Caniego}, M. and {Lubin}, P.~M. and {Mac{\'\i}as-P{\'e}rez}, J.~F. and {Maggio}, G. and {Maino}, D. and {Mandolesi}, N. and {Mangilli}, A. and {Marchini}, A. and {Maris}, M. and {Martin}, P.~G. and {Martinelli}, M. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Masi}, S. and {Matarrese}, S. and {McGehee}, P. and {Meinhold}, P.~R. and {Melchiorri}, A. and {Melin}, J. -B. and {Mendes}, L. and {Mennella}, A. and {Migliaccio}, M. and {Millea}, M. and {Mitra}, S. and {Miville-Desch{\^e}nes}, M. -A. and {Moneti}, A. and {Montier}, L. and {Morgante}, G. and {Mortlock}, D. and {Moss}, A. and {Munshi}, D. and {Murphy}, J.~A. and {Naselsky}, P. and {Nati}, F. and {Natoli}, P. and {Netterfield}, C.~B. and {N{\o}rgaard-Nielsen}, H.~U. and {Noviello}, F. and {Novikov}, D. and {Novikov}, I. and {Oxborrow}, C.~A. and {Paci}, F. and {Pagano}, L. and {Pajot}, F. and {Paladini}, R. and {Paoletti}, D. and {Partridge}, B. and {Pasian}, F. and {Patanchon}, G. and {Pearson}, T.~J. and {Perdereau}, O. and {Perotto}, L. and {Perrotta}, F. and {Pettorino}, V. and {Piacentini}, F. and {Piat}, M. and {Pierpaoli}, E. and {Pietrobon}, D. and {Plaszczynski}, S. and {Pointecouteau}, E. and {Polenta}, G. and {Popa}, L. and {Pratt}, G.~W. and {Pr{\'e}zeau}, G. and {Prunet}, S. and {Puget}, J. -L. and {Rachen}, J.~P. and {Reach}, W.~T. and {Rebolo}, R. and {Reinecke}, M. and {Remazeilles}, M. and {Renault}, C. and {Renzi}, A. and {Ristorcelli}, I. and {Rocha}, G. and {Rosset}, C. and {Rossetti}, M. and {Roudier}, G. and {Rouill{\'e} d'Orfeuil}, B. and {Rowan-Robinson}, M. and {Rubi{\~n}o-Mart{\'\i}n}, J.~A. and {Rusholme}, B. and {Said}, N. and {Salvatelli}, V. and {Salvati}, L. and {Sandri}, M. and {Santos}, D. and {Savelainen}, M. and {Savini}, G. and {Scott}, D. and {Seiffert}, M.~D. and {Serra}, P. and {Shellard}, E.~P.~S. and {Spencer}, L.~D. and {Spinelli}, M. and {Stolyarov}, V. and {Stompor}, R. and {Sudiwala}, R. and {Sunyaev}, R. and {Sutton}, D. and {Suur-Uski}, A. -S. and {Sygnet}, J. -F. and {Tauber}, J.~A. and {Terenzi}, L. and {Toffolatti}, L. and {Tomasi}, M. and {Tristram}, M. and {Trombetti}, T. and {Tucci}, M. and {Tuovinen}, J. and {T{\"u}rler}, M. and {Umana}, G. and {Valenziano}, L. and {Valiviita}, J. and {Van Tent}, F. and {Vielva}, P. and {Villa}, F. and {Wade}, L.~A. and {Wandelt}, B.~D. and {Wehus}, I.~K. and {White}, M. and {White}, S.~D.~M. and {Wilkinson}, A. and {Yvon}, D. and {Zacchei}, A. and {Zonca}, A.},
        title = "{Planck 2015 results. XIII. Cosmological parameters}",
      journal = {\aap},
     keywords = {cosmology: observations, cosmology: theory, cosmic background radiation, cosmological parameters, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2016,
        month = sep,
       volume = {594},
          eid = {A13},
        pages = {A13},
          doi = {10.1051/0004-6361/201525830},
archivePrefix = {arXiv},
       eprint = {1502.01589},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...594A..13P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Anomaliesl20,
       author = {{Vitenti}, Sandro D.~P. and {Peter}, Patrick and {Valentini}, Antony},
        title = "{Modeling the large-scale power deficit with smooth and discontinuous primordial spectra}",
      journal = {\prd},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2019,
        month = aug,
       volume = {100},
       number = {4},
          eid = {043506},
        pages = {043506},
          doi = {10.1103/PhysRevD.100.043506},
archivePrefix = {arXiv},
       eprint = {1901.08885},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019PhRvD.100d3506V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ReconParametrico1,
       author = {{Hazra}, Dhiraj Kumar and {Antony}, Akhil and {Shafieloo}, Arman},
        title = "{One spectrum to cure them all: signature from early Universe solves major anomalies and tensions in cosmology}",
      journal = {\jcap},
     keywords = {cosmological parameters from CMBR, cosmological perturbation theory, physics of the early universe, Astrophysics - Cosmology and Nongalactic Astrophysics, General Relativity and Quantum Cosmology, High Energy Physics - Theory},
         year = 2022,
        month = aug,
       volume = {2022},
       number = {8},
          eid = {063},
        pages = {063},
          doi = {10.1088/1475-7516/2022/08/063},
archivePrefix = {arXiv},
       eprint = {2201.12000},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022JCAP...08..063H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{FutureNonLinearDamping,
       author = {{Ballardini}, Mario and {Murgia}, Riccardo and {Baldi}, Marco and {Finelli}, Fabio and {Viel}, Matteo},
        title = "{Non-linear damping of superimposed primordial oscillations on the matter power spectrum in galaxy surveys}",
      journal = {\jcap},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = apr,
       volume = {2020},
       number = {4},
          eid = {030},
        pages = {030},
          doi = {10.1088/1475-7516/2020/04/030},
archivePrefix = {arXiv},
       eprint = {1912.12499},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020JCAP...04..030B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ModelInflationSpeedSound,
       author = {{Ca{\~n}as-Herrera}, Guadalupe and {Torrado}, Jes{\'u}s and {Ach{\'u}carro}, Ana},
        title = "{Bayesian reconstruction of the inflaton's speed of sound using CMB data}",
      journal = {\prd},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = jun,
       volume = {103},
       number = {12},
          eid = {123531},
        pages = {123531},
          doi = {10.1103/PhysRevD.103.123531},
archivePrefix = {arXiv},
       eprint = {2012.04640},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021PhRvD.103l3531C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{BayesianEvidencesPaper,
    author = {Trotta, Roberto},
    title = "{Applications of Bayesian model selection to cosmological parameters}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {378},
    number = {1},
    pages = {72-82},
    year = {2007},
    month = {05},
    abstract = "{Bayesian model selection is a tool for deciding whether the introduction of a new parameter is warranted by the data. I argue that the usual sampling statistic significance tests for a null hypothesis can be misleading, since they do not take into account the information gained through the data, when updating the prior distribution to the posterior. In contrast, Bayesian model selection offers a quantitative implementation of Occam's razor.I introduce the Savage–Dickey density ratio, a computationally quick method to determine the Bayes factor of two nested models and hence perform model selection. As an illustration, I consider three key parameters for our understanding of the cosmological concordance model. By using Wilkinson Microwave Anisotropy Probe (WMAP) 3-year data complemented by other cosmological measurements, I show that a non-scale-invariant spectral index of perturbations is favoured for any sensible choice of prior. It is also found that a flat universe is favoured with odds of 29:1 over non-flat models, and that there is strong evidence against a cold dark matter isocurvature component to the initial conditions which is totally (anti)correlated with the adiabatic mode (odds of about 2000:1), but that this is strongly dependent on the prior adopted.These results are contrasted with the analysis of WMAP 1-year data, which were not informative enough to allow a conclusion as to the status of the spectral index. In a companion paper, a new technique to forecast the Bayes factor of a future observation is presented.}",
    issn = {0035-8711},
    doi = {10.1111/j.1365-2966.2007.11738.x},
    url = {https://doi.org/10.1111/j.1365-2966.2007.11738.x},
    eprint = {https://academic.oup.com/mnras/article-pdf/378/1/72/3961005/mnras0378-0072.pdf},
}

@ARTICLE{ReconParametrico2,
       author = {{Antony}, Akhil and {Finelli}, Fabio and {Hazra}, Dhiraj Kumar and {Shafieloo}, Arman},
        title = "{Discordances in cosmology and the violation of slow-roll inflationary dynamics}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, General Relativity and Quantum Cosmology, High Energy Physics - Phenomenology, High Energy Physics - Theory},
         year = 2022,
        month = feb,
          eid = {arXiv:2202.14028},
        pages = {arXiv:2202.14028},
archivePrefix = {arXiv},
       eprint = {2202.14028},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022arXiv220214028A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ReconParametrico2LSS,
       author = {{Ballardini}, Mario and {Finelli}, Fabio},
        title = "{On the primordial origin of the smoothing excess in the $Planck$ temperature power spectrum in light of LSS data}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2022,
        month = jul,
          eid = {arXiv:2207.14410},
        pages = {arXiv:2207.14410},
archivePrefix = {arXiv},
       eprint = {2207.14410},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022arXiv220714410B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{SeoEisenstein,
       author = {{Seo}, Hee-Jong and {Eisenstein}, Daniel J.},
        title = "{Improved Forecasts for the Baryon Acoustic Oscillations and Cosmological Distance Scale}",
      journal = {\apj},
     keywords = {Cosmology: Cosmic Microwave Background, Cosmology: Cosmological Parameters, Cosmology: Distance Scale, Cosmology: Large-Scale Structure of Universe, Astrophysics},
         year = 2007,
        month = aug,
       volume = {665},
       number = {1},
        pages = {14-24},
          doi = {10.1086/519549},
archivePrefix = {arXiv},
       eprint = {astro-ph/0701079},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...665...14S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ReconModulationWMAP,
       author = {{Ichiki}, Kiyotomo and {Nagata}, Ryo and {Yokoyama}, Jun'Ichi},
        title = "{Cosmic discordance: Detection of a modulation in the primordial fluctuation spectrum}",
      journal = {\prd},
     keywords = {98.70.Vc, 95.30.-k, 98.80.Es, Background radiations, Fundamental aspects of astrophysics, Observational cosmology, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2010,
        month = apr,
       volume = {81},
       number = {8},
          eid = {083010},
        pages = {083010},
          doi = {10.1103/PhysRevD.81.083010},
archivePrefix = {arXiv},
       eprint = {0911.5108},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010PhRvD..81h3010I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{ReconFineStructure,
  title={Brute force reconstruction of the primordial fluctuation spectrum from five-year Wilkinson Microwave Anisotropy Probe observations},
  author={Kiyotomo Ichiki and Ryo Nagata},
  journal={Physical Review D},
  year={2009},
  volume={80},
  pages={083002}
}


@ARTICLE{LDModel,
       author = {{Lasenby}, Anthony and {Doran}, Chris},
        title = "{Closed universes, de Sitter space, and inflation}",
      journal = {\prd},
     keywords = {98.80.Cq, 04.20.Gz, 98.80.Es, 98.80.Jk, Particle-theory and field-theory models of the early Universe, Spacetime topology causal structure spinor structure, Observational cosmology, Mathematical and relativistic aspects of cosmology, Astrophysics, General Relativity and Quantum Cosmology},
         year = 2005,
        month = mar,
       volume = {71},
       number = {6},
          eid = {063502},
        pages = {063502},
          doi = {10.1103/PhysRevD.71.063502},
archivePrefix = {arXiv},
       eprint = {astro-ph/0307311},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005PhRvD..71f3502L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{JudgmentDayInflation,
       author = {{Chowdhury}, Debika and {Martin}, J{\'e}r{\^o}me and {Ringeval}, Christophe and {Vennin}, Vincent},
        title = "{Assessing the scientific status of inflation after Planck}",
      journal = {\prd},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, General Relativity and Quantum Cosmology, High Energy Physics - Phenomenology, High Energy Physics - Theory},
         year = 2019,
        month = oct,
       volume = {100},
       number = {8},
          eid = {083537},
        pages = {083537},
          doi = {10.1103/PhysRevD.100.083537},
archivePrefix = {arXiv},
       eprint = {1902.03951},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019PhRvD.100h3537C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{HiggsInflation,
       author = {{Bezrukov}, Fedor and {Shaposhnikov}, Mikhail},
        title = "{The Standard Model Higgs boson as the inflaton}",
      journal = {Physics Letters B},
     keywords = {98.80.Cq, 14.80.Bn, Particle-theory and field-theory models of the early Universe, Standard-model Higgs bosons, High Energy Physics - Theory, Astrophysics, High Energy Physics - Phenomenology},
         year = 2008,
        month = jan,
       volume = {659},
       number = {3},
        pages = {703-706},
          doi = {10.1016/j.physletb.2007.11.072},
archivePrefix = {arXiv},
       eprint = {0710.3755},
 primaryClass = {hep-th},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008PhLB..659..703B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{StarobinskiInflation,
       author = {{Starobinskii}, A.~A.},
        title = "{Spectrum of adiabatic perturbations in the universe in the presence of singularities in the inflation potential}",
      journal = {Pisma v Zhurnal Eksperimentalnoi i Teoreticheskoi Fiziki},
     keywords = {Adiabatic Conditions, Computational Astrophysics, Perturbation Theory, Universe, Cosmology, Inflating, Scalars, Astrophysics},
         year = 1992,
        month = may,
       volume = {55},
       number = {9-10},
        pages = {477-482},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1992PZETF..55..477S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{EnciclopediaInflation,
       author = {{Martin}, J{\'e}r{\^o}me and {Ringeval}, Christophe and {Vennin}, Vincent},
        title = "{Encyclop{\ae}dia Inflationaris}",
      journal = {Physics of the Dark Universe},
     keywords = {Cosmic inflation, Slow-roll, Reheating, Cosmic Microwave Background, ASPIC, Astrophysics - Cosmology and Nongalactic Astrophysics, General Relativity and Quantum Cosmology, High Energy Physics - Phenomenology, High Energy Physics - Theory},
         year = 2014,
        month = dec,
       volume = {5},
        pages = {75-235},
          doi = {10.1016/j.dark.2014.01.003},
archivePrefix = {arXiv},
       eprint = {1303.3787},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014PDU.....5...75M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{AnalyticAproachNonSlowRoll,
       author = {{Tasinato}, Gianmassimo},
        title = "{Analytic approach to non-slow-roll inflation}",
      journal = {\prd},
     keywords = {High Energy Physics - Theory, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = jan,
       volume = {103},
       number = {2},
          eid = {023535},
        pages = {023535},
          doi = {10.1103/PhysRevD.103.023535},
archivePrefix = {arXiv},
       eprint = {2012.02518},
 primaryClass = {hep-th},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021PhRvD.103b3535T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book{Jeffreys1998theory,
  title={The Theory of Probability},
  author={Jeffreys, H.},
  isbn={9780191589676},
  series={Oxford Classic Texts in the Physical Sciences},
  url={https://books.google.it/books?id=vh9Act9rtzQC},
  year={1998},
  publisher={OUP Oxford}
}

@ARTICLE{CAMB,
       author = {{Lewis}, Antony and {Challinor}, Anthony and {Lasenby}, Anthony},
        title = "{Efficient Computation of Cosmic Microwave Background Anisotropies in Closed Friedmann-Robertson-Walker Models}",
      journal = {\apj},
     keywords = {Cosmology: Cosmic Microwave Background, Cosmology: Theory, Astrophysics},
         year = 2000,
        month = aug,
       volume = {538},
       number = {2},
        pages = {473-476},
          doi = {10.1086/309179},
archivePrefix = {arXiv},
       eprint = {astro-ph/9911177},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...538..473L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{SDSSDR04,
       author = {{Adelman-McCarthy}, Jennifer K. and {Ag{\"u}eros}, Marcel A. and {Allam}, Sahar S. and {Anderson}, Kurt S.~J. and {Anderson}, Scott F. and {Annis}, James and {Bahcall}, Neta A. and {Baldry}, Ivan K. and {Barentine}, J.~C. and {Berlind}, Andreas and {Bernardi}, Mariangela and {Blanton}, Michael R. and {Boroski}, William N. and {Brewington}, Howard J. and {Brinchmann}, Jarle and {Brinkmann}, J. and {Brunner}, Robert J. and {Budav{\'a}ri}, Tam{\'a}s and {Carey}, Larry N. and {Carr}, Michael A. and {Castander}, Francisco J. and {Connolly}, A.~J. and {Csabai}, Istv{\'a}n and {Czarapata}, Paul C. and {Dalcanton}, Julianne J. and {Doi}, Mamoru and {Dong}, Feng and {Eisenstein}, Daniel J. and {Evans}, Michael L. and {Fan}, Xiaohui and {Finkbeiner}, Douglas P. and {Friedman}, Scott D. and {Frieman}, Joshua A. and {Fukugita}, Masataka and {Gillespie}, Bruce and {Glazebrook}, Karl and {Gray}, Jim and {Grebel}, Eva K. and {Gunn}, James E. and {Gurbani}, Vijay K. and {de Haas}, Ernst and {Hall}, Patrick B. and {Harris}, Frederick H. and {Harvanek}, Michael and {Hawley}, Suzanne L. and {Hayes}, Jeffrey and {Hendry}, John S. and {Hennessy}, Gregory S. and {Hindsley}, Robert B. and {Hirata}, Christopher M. and {Hogan}, Craig J. and {Hogg}, David W. and {Holmgren}, Donald J. and {Holtzman}, Jon A. and {Ichikawa}, Shin-ichi and {Ivezi{\'c}}, {\v{Z}}eljko and {Jester}, Sebastian and {Johnston}, David E. and {Jorgensen}, Anders M. and {Juri{\'c}}, Mario and {Kent}, Stephen M. and {Kleinman}, S.~J. and {Knapp}, G.~R. and {Kniazev}, Alexei Yu. and {Kron}, Richard G. and {Krzesinski}, Jurek and {Kuropatkin}, Nikolay and {Lamb}, Donald Q. and {Lampeitl}, Hubert and {Lee}, Brian C. and {Leger}, R. French and {Lin}, Huan and {Long}, Daniel C. and {Loveday}, Jon and {Lupton}, Robert H. and {Margon}, Bruce and {Mart{\'\i}nez-Delgado}, David and {Mandelbaum}, Rachel and {Matsubara}, Takahiko and {McGehee}, Peregrine M. and {McKay}, Timothy A. and {Meiksin}, Avery and {Munn}, Jeffrey A. and {Nakajima}, Reiko and {Nash}, Thomas and {Neilsen}, Eric H., Jr. and {Newberg}, Heidi Jo and {Newman}, Peter R. and {Nichol}, Robert C. and {Nicinski}, Tom and {Nieto-Santisteban}, Maria and {Nitta}, Atsuko and {O'Mullane}, William and {Okamura}, Sadanori and {Owen}, Russell and {Padmanabhan}, Nikhil and {Pauls}, George and {Peoples}, John, Jr. and {Pier}, Jeffrey R. and {Pope}, Adrian C. and {Pourbaix}, Dimitri and {Quinn}, Thomas R. and {Richards}, Gordon T. and {Richmond}, Michael W. and {Rockosi}, Constance M. and {Schlegel}, David J. and {Schneider}, Donald P. and {Schroeder}, Joshua and {Scranton}, Ryan and {Seljak}, Uro{\v{s}} and {Sheldon}, Erin and {Shimasaku}, Kazu and {Smith}, J. Allyn and {Smol{\v{c}}i{\'c}}, Vernesa and {Snedden}, Stephanie A. and {Stoughton}, Chris and {Strauss}, Michael A. and {SubbaRao}, Mark and {Szalay}, Alexander S. and {Szapudi}, Istv{\'a}n and {Szkody}, Paula and {Tegmark}, Max and {Thakar}, Aniruddha R. and {Tucker}, Douglas L. and {Uomoto}, Alan and {Vanden Berk}, Daniel E. and {Vandenberg}, Jan and {Vogeley}, Michael S. and {Voges}, Wolfgang and {Vogt}, Nicole P. and {Walkowicz}, Lucianne M. and {Weinberg}, David H. and {West}, Andrew A. and {White}, Simon D.~M. and {Xu}, Yongzhong and {Yanny}, Brian and {Yocum}, D.~R. and {York}, Donald G. and {Zehavi}, Idit and {Zibetti}, Stefano and {Zucker}, Daniel B.},
        title = "{The Fourth Data Release of the Sloan Digital Sky Survey}",
      journal = {\apjs},
     keywords = {Atlases, Catalogs, Surveys, Astrophysics},
         year = 2006,
        month = jan,
       volume = {162},
       number = {1},
        pages = {38-48},
          doi = {10.1086/497917},
archivePrefix = {arXiv},
       eprint = {astro-ph/0507711},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJS..162...38A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DensitiesOriginal,
       author = {{Efstathiou}, G. and {Bernstein}, G. and {Katz}, N. and {Tyson}, J.~A. and {Guhathakurta}, P.},
        title = "{The Clustering of Faint Galaxies}",
      journal = {\apjl},
     keywords = {Faint Objects, Galactic Clusters, Galactic Evolution, Angular Correlation, Astronomical Models, Charge Coupled Devices, Astrophysics, COSMOLOGY, GALAXIES: CLUSTERING, GALAXIES: FORMATION},
         year = 1991,
        month = oct,
       volume = {380},
        pages = {L47},
          doi = {10.1086/186170},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1991ApJ...380L..47E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{EuclidSpecifications,
       author = {{Laureijs}, R. and {Amiaux}, J. and {Arduini}, S. and {Augu{\`e}res}, J. -L. and {Brinchmann}, J. and {Cole}, R. and {Cropper}, M. and {Dabin}, C. and {Duvet}, L. and {Ealet}, A. and {Garilli}, B. and {Gondoin}, P. and {Guzzo}, L. and {Hoar}, J. and {Hoekstra}, H. and {Holmes}, R. and {Kitching}, T. and {Maciaszek}, T. and {Mellier}, Y. and {Pasian}, F. and {Percival}, W. and {Rhodes}, J. and {Saavedra Criado}, G. and {Sauvage}, M. and {Scaramella}, R. and {Valenziano}, L. and {Warren}, S. and {Bender}, R. and {Castander}, F. and {Cimatti}, A. and {Le F{\`e}vre}, O. and {Kurki-Suonio}, H. and {Levi}, M. and {Lilje}, P. and {Meylan}, G. and {Nichol}, R. and {Pedersen}, K. and {Popa}, V. and {Rebolo Lopez}, R. and {Rix}, H. -W. and {Rottgering}, H. and {Zeilinger}, W. and {Grupp}, F. and {Hudelot}, P. and {Massey}, R. and {Meneghetti}, M. and {Miller}, L. and {Paltani}, S. and {Paulin-Henriksson}, S. and {Pires}, S. and {Saxton}, C. and {Schrabback}, T. and {Seidel}, G. and {Walsh}, J. and {Aghanim}, N. and {Amendola}, L. and {Bartlett}, J. and {Baccigalupi}, C. and {Beaulieu}, J. -P. and {Benabed}, K. and {Cuby}, J. -G. and {Elbaz}, D. and {Fosalba}, P. and {Gavazzi}, G. and {Helmi}, A. and {Hook}, I. and {Irwin}, M. and {Kneib}, J. -P. and {Kunz}, M. and {Mannucci}, F. and {Moscardini}, L. and {Tao}, C. and {Teyssier}, R. and {Weller}, J. and {Zamorani}, G. and {Zapatero Osorio}, M.~R. and {Boulade}, O. and {Foumond}, J.~J. and {Di Giorgio}, A. and {Guttridge}, P. and {James}, A. and {Kemp}, M. and {Martignac}, J. and {Spencer}, A. and {Walton}, D. and {Bl{\"u}mchen}, T. and {Bonoli}, C. and {Bortoletto}, F. and {Cerna}, C. and {Corcione}, L. and {Fabron}, C. and {Jahnke}, K. and {Ligori}, S. and {Madrid}, F. and {Martin}, L. and {Morgante}, G. and {Pamplona}, T. and {Prieto}, E. and {Riva}, M. and {Toledo}, R. and {Trifoglio}, M. and {Zerbi}, F. and {Abdalla}, F. and {Douspis}, M. and {Grenet}, C. and {Borgani}, S. and {Bouwens}, R. and {Courbin}, F. and {Delouis}, J. -M. and {Dubath}, P. and {Fontana}, A. and {Frailis}, M. and {Grazian}, A. and {Koppenh{\"o}fer}, J. and {Mansutti}, O. and {Melchior}, M. and {Mignoli}, M. and {Mohr}, J. and {Neissner}, C. and {Noddle}, K. and {Poncet}, M. and {Scodeggio}, M. and {Serrano}, S. and {Shane}, N. and {Starck}, J. -L. and {Surace}, C. and {Taylor}, A. and {Verdoes-Kleijn}, G. and {Vuerli}, C. and {Williams}, O.~R. and {Zacchei}, A. and {Altieri}, B. and {Escudero Sanz}, I. and {Kohley}, R. and {Oosterbroek}, T. and {Astier}, P. and {Bacon}, D. and {Bardelli}, S. and {Baugh}, C. and {Bellagamba}, F. and {Benoist}, C. and {Bianchi}, D. and {Biviano}, A. and {Branchini}, E. and {Carbone}, C. and {Cardone}, V. and {Clements}, D. and {Colombi}, S. and {Conselice}, C. and {Cresci}, G. and {Deacon}, N. and {Dunlop}, J. and {Fedeli}, C. and {Fontanot}, F. and {Franzetti}, P. and {Giocoli}, C. and {Garcia-Bellido}, J. and {Gow}, J. and {Heavens}, A. and {Hewett}, P. and {Heymans}, C. and {Holland}, A. and {Huang}, Z. and {Ilbert}, O. and {Joachimi}, B. and {Jennins}, E. and {Kerins}, E. and {Kiessling}, A. and {Kirk}, D. and {Kotak}, R. and {Krause}, O. and {Lahav}, O. and {van Leeuwen}, F. and {Lesgourgues}, J. and {Lombardi}, M. and {Magliocchetti}, M. and {Maguire}, K. and {Majerotto}, E. and {Maoli}, R. and {Marulli}, F. and {Maurogordato}, S. and {McCracken}, H. and {McLure}, R. and {Melchiorri}, A. and {Merson}, A. and {Moresco}, M. and {Nonino}, M. and {Norberg}, P. and {Peacock}, J. and {Pello}, R. and {Penny}, M. and {Pettorino}, V. and {Di Porto}, C. and {Pozzetti}, L. and {Quercellini}, C. and {Radovich}, M. and {Rassat}, A. and {Roche}, N. and {Ronayette}, S. and {Rossetti}, E. and {Sartoris}, B. and {Schneider}, P. and {Semboloni}, E. and {Serjeant}, S. and {Simpson}, F. and {Skordis}, C. and {Smadja}, G. and {Smartt}, S. and {Spano}, P. and {Spiro}, S. and {Sullivan}, M. and {Tilquin}, A. and {Trotta}, R. and {Verde}, L. and {Wang}, Y. and {Williger}, G. and {Zhao}, G. and {Zoubian}, J. and {Zucca}, E.},
        title = "{Euclid Definition Study Report}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Extragalactic Astrophysics, Astrophysics - Galaxy Astrophysics},
         year = 2011,
        month = oct,
          eid = {arXiv:1110.3193},
        pages = {arXiv:1110.3193},
archivePrefix = {arXiv},
       eprint = {1110.3193},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011arXiv1110.3193L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DESISpecifications,
       author = {{DESI Collaboration} and {Aghamousa}, Amir and {Aguilar}, Jessica and {Ahlen}, Steve and {Alam}, Shadab and {Allen}, Lori E. and {Allende Prieto}, Carlos and {Annis}, James and {Bailey}, Stephen and {Balland}, Christophe and {Ballester}, Otger and {Baltay}, Charles and {Beaufore}, Lucas and {Bebek}, Chris and {Beers}, Timothy C. and {Bell}, Eric F. and {Bernal}, Jos{\'e} Luis and {Besuner}, Robert and {Beutler}, Florian and {Blake}, Chris and {Bleuler}, Hannes and {Blomqvist}, Michael and {Blum}, Robert and {Bolton}, Adam S. and {Briceno}, Cesar and {Brooks}, David and {Brownstein}, Joel R. and {Buckley-Geer}, Elizabeth and {Burden}, Angela and {Burtin}, Etienne and {Busca}, Nicolas G. and {Cahn}, Robert N. and {Cai}, Yan-Chuan and {Cardiel-Sas}, Laia and {Carlberg}, Raymond G. and {Carton}, Pierre-Henri and {Casas}, Ricard and {Castander}, Francisco J. and {Cervantes-Cota}, Jorge L. and {Claybaugh}, Todd M. and {Close}, Madeline and {Coker}, Carl T. and {Cole}, Shaun and {Comparat}, Johan and {Cooper}, Andrew P. and {Cousinou}, M. -C. and {Crocce}, Martin and {Cuby}, Jean-Gabriel and {Cunningham}, Daniel P. and {Davis}, Tamara M. and {Dawson}, Kyle S. and {de la Macorra}, Axel and {De Vicente}, Juan and {Delubac}, Timoth{\'e}e and {Derwent}, Mark and {Dey}, Arjun and {Dhungana}, Govinda and {Ding}, Zhejie and {Doel}, Peter and {Duan}, Yutong T. and {Ealet}, Anne and {Edelstein}, Jerry and {Eftekharzadeh}, Sarah and {Eisenstein}, Daniel J. and {Elliott}, Ann and {Escoffier}, St{\'e}phanie and {Evatt}, Matthew and {Fagrelius}, Parker and {Fan}, Xiaohui and {Fanning}, Kevin and {Farahi}, Arya and {Farihi}, Jay and {Favole}, Ginevra and {Feng}, Yu and {Fernandez}, Enrique and {Findlay}, Joseph R. and {Finkbeiner}, Douglas P. and {Fitzpatrick}, Michael J. and {Flaugher}, Brenna and {Flender}, Samuel and {Font-Ribera}, Andreu and {Forero-Romero}, Jaime E. and {Fosalba}, Pablo and {Frenk}, Carlos S. and {Fumagalli}, Michele and {Gaensicke}, Boris T. and {Gallo}, Giuseppe and {Garcia-Bellido}, Juan and {Gaztanaga}, Enrique and {Pietro Gentile Fusillo}, Nicola and {Gerard}, Terry and {Gershkovich}, Irena and {Giannantonio}, Tommaso and {Gillet}, Denis and {Gonzalez-de-Rivera}, Guillermo and {Gonzalez-Perez}, Violeta and {Gott}, Shelby and {Graur}, Or and {Gutierrez}, Gaston and {Guy}, Julien and {Habib}, Salman and {Heetderks}, Henry and {Heetderks}, Ian and {Heitmann}, Katrin and {Hellwing}, Wojciech A. and {Herrera}, David A. and {Ho}, Shirley and {Holland}, Stephen and {Honscheid}, Klaus and {Huff}, Eric and {Hutchinson}, Timothy A. and {Huterer}, Dragan and {Hwang}, Ho Seong and {Illa Laguna}, Joseph Maria and {Ishikawa}, Yuzo and {Jacobs}, Dianna and {Jeffrey}, Niall and {Jelinsky}, Patrick and {Jennings}, Elise and {Jiang}, Linhua and {Jimenez}, Jorge and {Johnson}, Jennifer and {Joyce}, Richard and {Jullo}, Eric and {Juneau}, St{\'e}phanie and {Kama}, Sami and {Karcher}, Armin and {Karkar}, Sonia and {Kehoe}, Robert and {Kennamer}, Noble and {Kent}, Stephen and {Kilbinger}, Martin and {Kim}, Alex G. and {Kirkby}, David and {Kisner}, Theodore and {Kitanidis}, Ellie and {Kneib}, Jean-Paul and {Koposov}, Sergey and {Kovacs}, Eve and {Koyama}, Kazuya and {Kremin}, Anthony and {Kron}, Richard and {Kronig}, Luzius and {Kueter-Young}, Andrea and {Lacey}, Cedric G. and {Lafever}, Robin and {Lahav}, Ofer and {Lambert}, Andrew and {Lampton}, Michael and {Landriau}, Martin and {Lang}, Dustin and {Lauer}, Tod R. and {Le Goff}, Jean-Marc and {Le Guillou}, Laurent and {Le Van Suu}, Auguste and {Lee}, Jae Hyeon and {Lee}, Su-Jeong and {Leitner}, Daniela and {Lesser}, Michael and {Levi}, Michael E. and {L'Huillier}, Benjamin and {Li}, Baojiu and {Liang}, Ming and {Lin}, Huan and {Linder}, Eric and {Loebman}, Sarah R. and {Luki{\'c}}, Zarija and {Ma}, Jun and {MacCrann}, Niall and {Magneville}, Christophe and {Makarem}, Laleh and {Manera}, Marc and {Manser}, Christopher J. and {Marshall}, Robert and {Martini}, Paul and {Massey}, Richard and {Matheson}, Thomas and {McCauley}, Jeremy and {McDonald}, Patrick and {McGreer}, Ian D. and {Meisner}, Aaron and {Metcalfe}, Nigel and {Miller}, Timothy N. and {Miquel}, Ramon and {Moustakas}, John and {Myers}, Adam and {Naik}, Milind and {Newman}, Jeffrey A. and {Nichol}, Robert C. and {Nicola}, Andrina and {Nicolati da Costa}, Luiz and {Nie}, Jundan and {Niz}, Gustavo and {Norberg}, Peder and {Nord}, Brian and {Norman}, Dara and {Nugent}, Peter and {O'Brien}, Thomas and {Oh}, Minji and {Olsen}, Knut A.~G. and {Padilla}, Cristobal and {Padmanabhan}, Hamsa and {Padmanabhan}, Nikhil and {Palanque-Delabrouille}, Nathalie and {Palmese}, Antonella and {Pappalardo}, Daniel and {P{\^a}ris}, Isabelle and {Park}, Changbom and {Patej}, Anna and {Peacock}, John A. and {Peiris}, Hiranya V. and {Peng}, Xiyan and {Percival}, Will J. and {Perruchot}, Sandrine and {Pieri}, Matthew M. and {Pogge}, Richard and {Pollack}, Jennifer E. and {Poppett}, Claire and {Prada}, Francisco and {Prakash}, Abhishek and {Probst}, Ronald G. and {Rabinowitz}, David and {Raichoor}, Anand and {Ree}, Chang Hee and {Refregier}, Alexandre and {Regal}, Xavier and {Reid}, Beth and {Reil}, Kevin and {Rezaie}, Mehdi and {Rockosi}, Constance M. and {Roe}, Natalie and {Ronayette}, Samuel and {Roodman}, Aaron and {Ross}, Ashley J. and {Ross}, Nicholas P. and {Rossi}, Graziano and {Rozo}, Eduardo and {Ruhlmann-Kleider}, Vanina and {Rykoff}, Eli S. and {Sabiu}, Cristiano and {Samushia}, Lado and {Sanchez}, Eusebio and {Sanchez}, Javier and {Schlegel}, David J. and {Schneider}, Michael and {Schubnell}, Michael and {Secroun}, Aur{\'e}lia and {Seljak}, Uros and {Seo}, Hee-Jong and {Serrano}, Santiago and {Shafieloo}, Arman and {Shan}, Huanyuan and {Sharples}, Ray and {Sholl}, Michael J. and {Shourt}, William V. and {Silber}, Joseph H. and {Silva}, David R. and {Sirk}, Martin M. and {Slosar}, Anze and {Smith}, Alex and {Smoot}, George F. and {Som}, Debopam and {Song}, Yong-Seon and {Sprayberry}, David and {Staten}, Ryan and {Stefanik}, Andy and {Tarle}, Gregory and {Sien Tie}, Suk and {Tinker}, Jeremy L. and {Tojeiro}, Rita and {Valdes}, Francisco and {Valenzuela}, Octavio and {Valluri}, Monica and {Vargas-Magana}, Mariana and {Verde}, Licia and {Walker}, Alistair R. and {Wang}, Jiali and {Wang}, Yuting and {Weaver}, Benjamin A. and {Weaverdyck}, Curtis and {Wechsler}, Risa H. and {Weinberg}, David H. and {White}, Martin and {Yang}, Qian and {Yeche}, Christophe and {Zhang}, Tianmeng and {Zhao}, Gong-Bo and {Zheng}, Yi and {Zhou}, Xu and {Zhou}, Zhimin and {Zhu}, Yaling and {Zou}, Hu and {Zu}, Ying},
        title = "{The DESI Experiment Part I: Science,Targeting, and Survey Design}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2016,
        month = oct,
          eid = {arXiv:1611.00036},
        pages = {arXiv:1611.00036},
archivePrefix = {arXiv},
       eprint = {1611.00036},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016arXiv161100036D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{JPASSpecifications,
       author = {{Benitez}, N. and {Dupke}, R. and {Moles}, M. and {Sodre}, L. and {Cenarro}, J. and {Marin-Franch}, A. and {Taylor}, K. and {Cristobal}, D. and {Fernandez-Soto}, A. and {Mendes de Oliveira}, C. and {Cepa-Nogue}, J. and {Abramo}, L.~R. and {Alcaniz}, J.~S. and {Overzier}, R. and {Hernandez-Monteagudo}, C. and {Alfaro}, E.~J. and {Kanaan}, A. and {Carvano}, J.~M. and {Reis}, R.~R.~R. and {Martinez Gonzalez}, E. and {Ascaso}, B. and {Ballesteros}, F. and {Xavier}, H.~S. and {Varela}, J. and {Ederoclite}, A. and {Vazquez Ramio}, H. and {Broadhurst}, T. and {Cypriano}, E. and {Angulo}, R. and {Diego}, J.~M. and {Zandivarez}, A. and {Diaz}, E. and {Melchior}, P. and {Umetsu}, K. and {Spinelli}, P.~F. and {Zitrin}, A. and {Coe}, D. and {Yepes}, G. and {Vielva}, P. and {Sahni}, V. and {Marcos-Caballero}, A. and {Shu Kitaura}, F. and {Maroto}, A.~L. and {Masip}, M. and {Tsujikawa}, S. and {Carneiro}, S. and {Gonzalez Nuevo}, J. and {Carvalho}, G.~C. and {Reboucas}, M.~J. and {Carvalho}, J.~C. and {Abdalla}, E. and {Bernui}, A. and {Pigozzo}, C. and {Ferreira}, E.~G.~M. and {Chandrachani Devi}, N. and {Bengaly}, C.~A.~P., Jr. and {Campista}, M. and {Amorim}, A. and {Asari}, N.~V. and {Bongiovanni}, A. and {Bonoli}, S. and {Bruzual}, G. and {Cardiel}, N. and {Cava}, A. and {Cid Fernandes}, R. and {Coelho}, P. and {Cortesi}, A. and {Delgado}, R.~G. and {Diaz Garcia}, L. and {Espinosa}, J.~M.~R. and {Galliano}, E. and {Gonzalez-Serrano}, J.~I. and {Falcon-Barroso}, J. and {Fritz}, J. and {Fernandes}, C. and {Gorgas}, J. and {Hoyos}, C. and {Jimenez-Teja}, Y. and {Lopez-Aguerri}, J.~A. and {Lopez-San Juan}, C. and {Mateus}, A. and {Molino}, A. and {Novais}, P. and {OMill}, A. and {Oteo}, I. and {Perez-Gonzalez}, P.~G. and {Poggianti}, B. and {Proctor}, R. and {Ricciardelli}, E. and {Sanchez-Blazquez}, P. and {Storchi-Bergmann}, T. and {Telles}, E. and {Schoennell}, W. and {Trujillo}, N. and {Vazdekis}, A. and {Viironen}, K. and {Daflon}, S. and {Aparicio-Villegas}, T. and {Rocha}, D. and {Ribeiro}, T. and {Borges}, M. and {Martins}, S.~L. and {Marcolino}, W. and {Martinez-Delgado}, D. and {Perez-Torres}, M.~A. and {Siffert}, B.~B. and {Calvao}, M.~O. and {Sako}, M. and {Kessler}, R. and {Alvarez-Candal}, A. and {De Pra}, M. and {Roig}, F. and {Lazzaro}, D. and {Gorosabel}, J. and {Lopes de Oliveira}, R. and {Lima-Neto}, G.~B. and {Irwin}, J. and {Liu}, J.~F. and {Alvarez}, E. and {Balmes}, I. and {Chueca}, S. and {Costa-Duarte}, M.~V. and {da Costa}, A.~A. and {Dantas}, M.~L.~L. and {Diaz}, A.~Y. and {Fabregat}, J. and {Ferrari}, F. and {Gavela}, B. and {Gracia}, S.~G. and {Gruel}, N. and {Gutierrez}, J.~L.~L. and {Guzman}, R. and {Hernandez-Fernandez}, J.~D. and {Herranz}, D. and {Hurtado-Gil}, L. and {Jablonsky}, F. and {Laporte}, R. and {Le Tiran}, L.~L. and {Licandro}, J and {Lima}, M. and {Martin}, E. and {Martinez}, V. and {Montero}, J.~J.~C. and {Penteado}, P. and {Pereira}, C.~B. and {Peris}, V. and {Quilis}, V. and {Sanchez-Portal}, M. and {Soja}, A.~C. and {Solano}, E. and {Torra}, J. and {Valdivielso}, L.},
        title = "{J-PAS: The Javalambre-Physics of the Accelerated Universe Astrophysical Survey}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2014,
        month = mar,
          eid = {arXiv:1403.5237},
        pages = {arXiv:1403.5237},
archivePrefix = {arXiv},
       eprint = {1403.5237},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014arXiv1403.5237B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{BiasHighZ,
       author = {{Ross}, Nicholas P. and {Shen}, Yue,and {Strauss}, Michael A. and {Vanden Berk}, Daniel E. and {Connolly}, Andrew J. and {Richards}, Gordon T. and {Schneider}, Donald P. and {Weinberg}, David H. and {Hall}, Patrick B. and {Bahcall}, Neta A. and {Brunner},Robert J.},
        title = "{Clustering of Low-redshift (z $<=$ 2.2) Quasars from the Sloan Digital Sky Survey}",
      journal = {\apj},
     keywords = {cosmology: observations, large-scale structure of universe, quasars: general, surveys, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2009,
        month = jun,
       volume = {697},
       number = {2},
        pages = {1634-1655},
          doi = {10.1088/0004-637X/697/2/1634},
archivePrefix = {arXiv},
       eprint = {0903.3230},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...697.1634R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CovarianceMatrix,
       author = {{Carron}, J. and {Wolk}, M. and {Szapudi}, I.},
        title = "{On the information content of the matter power spectrum}",
      journal = {\mnras},
     keywords = {methods: analytical, methods: statistical, cosmological parameters, large-scale structure of Universe, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2015,
        month = oct,
       volume = {453},
       number = {1},
        pages = {450-455},
          doi = {10.1093/mnras/stv1595},
archivePrefix = {arXiv},
       eprint = {1412.5511},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.453..450C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{BiasLowZ,
       author = {{Ross}, Nicholas P. and {Shen}, Yue and {Strauss}, Michael A. and {Vanden Berk}, Daniel E. and {Connolly}, Andrew J. and {Richards}, Gordon T. and {Schneider}, Donald P. and {Weinberg}, David H. and {Hall}, Patrick B. and {Bahcall}, Neta A. and {Brunner}, Robert J.},
        title = "{Clustering of Low-redshift (z <= 2.2) Quasars from the Sloan Digital Sky Survey}",
      journal = {\apj},
     keywords = {cosmology: observations, large-scale structure of universe, quasars: general, surveys, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2009,
        month = jun,
       volume = {697},
       number = {2},
        pages = {1634-1655},
          doi = {10.1088/0004-637X/697/2/1634},
archivePrefix = {arXiv},
       eprint = {0903.3230},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...697.1634R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{SDSSIIIBOSS,
       author = {{Eisenstein}, Daniel J. and {Weinberg}, David H. and {Agol}, Eric and {Aihara}, Hiroaki and {Allende Prieto}, Carlos and {Anderson}, Scott F. and {Arns}, James A. and {Aubourg}, {\'E}ric and {Bailey}, Stephen and {Balbinot}, Eduardo and {Barkhouser}, Robert and {Beers}, Timothy C. and {Berlind}, Andreas A. and {Bickerton}, Steven J. and {Bizyaev}, Dmitry and {Blanton}, Michael R. and {Bochanski}, John J. and {Bolton}, Adam S. and {Bosman}, Casey T. and {Bovy}, Jo and {Brandt}, W.~N. and {Breslauer}, Ben and {Brewington}, Howard J. and {Brinkmann}, J. and {Brown}, Peter J. and {Brownstein}, Joel R. and {Burger}, Dan and {Busca}, Nicolas G. and {Campbell}, Heather and {Cargile}, Phillip A. and {Carithers}, William C. and {Carlberg}, Joleen K. and {Carr}, Michael A. and {Chang}, Liang and {Chen}, Yanmei and {Chiappini}, Cristina and {Comparat}, Johan and {Connolly}, Natalia and {Cortes}, Marina and {Croft}, Rupert A.~C. and {Cunha}, Katia and {da Costa}, Luiz N. and {Davenport}, James R.~A. and {Dawson}, Kyle and {De Lee}, Nathan and {Porto de Mello}, Gustavo F. and {de Simoni}, Fernando and {Dean}, Janice and {Dhital}, Saurav and {Ealet}, Anne and {Ebelke}, Garrett L. and {Edmondson}, Edward M. and {Eiting}, Jacob M. and {Escoffier}, Stephanie and {Esposito}, Massimiliano and {Evans}, Michael L. and {Fan}, Xiaohui and {Femen{\'\i}a Castell{\'a}}, Bruno and {Dutra Ferreira}, Leticia and {Fitzgerald}, Greg and {Fleming}, Scott W. and {Font-Ribera}, Andreu and {Ford}, Eric B. and {Frinchaboy}, Peter M. and {Garc{\'\i}a P{\'e}rez}, Ana Elia and {Gaudi}, B. Scott and {Ge}, Jian and {Ghezzi}, Luan and {Gillespie}, Bruce A. and {Gilmore}, G. and {Girardi}, L{\'e}o and {Gott}, J. Richard and {Gould}, Andrew and {Grebel}, Eva K. and {Gunn}, James E. and {Hamilton}, Jean-Christophe and {Harding}, Paul and {Harris}, David W. and {Hawley}, Suzanne L. and {Hearty}, Frederick R. and {Hennawi}, Joseph F. and {Gonz{\'a}lez Hern{\'a}ndez}, Jonay I. and {Ho}, Shirley and {Hogg}, David W. and {Holtzman}, Jon A. and {Honscheid}, Klaus and {Inada}, Naohisa and {Ivans}, Inese I. and {Jiang}, Linhua and {Jiang}, Peng and {Johnson}, Jennifer A. and {Jordan}, Cathy and {Jordan}, Wendell P. and {Kauffmann}, Guinevere and {Kazin}, Eyal and {Kirkby}, David and {Klaene}, Mark A. and {Knapp}, G.~R. and {Kneib}, Jean-Paul and {Kochanek}, C.~S. and {Koesterke}, Lars and {Kollmeier}, Juna A. and {Kron}, Richard G. and {Lampeitl}, Hubert and {Lang}, Dustin and {Lawler}, James E. and {Le Goff}, Jean-Marc and {Lee}, Brian L. and {Lee}, Young Sun and {Leisenring}, Jarron M. and {Lin}, Yen-Ting and {Liu}, Jian and {Long}, Daniel C. and {Loomis}, Craig P. and {Lucatello}, Sara and {Lundgren}, Britt and {Lupton}, Robert H. and {Ma}, Bo and {Ma}, Zhibo and {MacDonald}, Nicholas and {Mack}, Claude and {Mahadevan}, Suvrath and {Maia}, Marcio A.~G. and {Majewski}, Steven R. and {Makler}, Martin and {Malanushenko}, Elena and {Malanushenko}, Viktor and {Mandelbaum}, Rachel and {Maraston}, Claudia and {Margala}, Daniel and {Maseman}, Paul and {Masters}, Karen L. and {McBride}, Cameron K. and {McDonald}, Patrick and {McGreer}, Ian D. and {McMahon}, Richard G. and {Mena Requejo}, Olga and {M{\'e}nard}, Brice and {Miralda-Escud{\'e}}, Jordi and {Morrison}, Heather L. and {Mullally}, Fergal and {Muna}, Demitri and {Murayama}, Hitoshi and {Myers}, Adam D. and {Naugle}, Tracy and {Neto}, Angelo Fausti and {Nguyen}, Duy Cuong and {Nichol}, Robert C. and {Nidever}, David L. and {O'Connell}, Robert W. and {Ogando}, Ricardo L.~C. and {Olmstead}, Matthew D. and {Oravetz}, Daniel J. and {Padmanabhan}, Nikhil and {Paegert}, Martin and {Palanque-Delabrouille}, Nathalie and {Pan}, Kaike and {Pandey}, Parul and {Parejko}, John K. and {P{\^a}ris}, Isabelle and {Pellegrini}, Paulo and {Pepper}, Joshua and {Percival}, Will J. and {Petitjean}, Patrick and {Pfaffenberger}, Robert and {Pforr}, Janine and {Phleps}, Stefanie and {Pichon}, Christophe and {Pieri}, Matthew M. and {Prada}, Francisco and {Price-Whelan}, Adrian M. and {Raddick}, M. Jordan and {Ramos}, Beatriz H.~F. and {Reid}, I. Neill and {Reyle}, Celine and {Rich}, James and {Richards}, Gordon T. and {Rieke}, George H. and {Rieke}, Marcia J. and {Rix}, Hans-Walter and {Robin}, Annie C. and {Rocha-Pinto}, Helio J. and {Rockosi}, Constance M. and {Roe}, Natalie A. and {Rollinde}, Emmanuel and {Ross}, Ashley J. and {Ross}, Nicholas P. and {Rossetto}, Bruno and {S{\'a}nchez}, Ariel G. and {Santiago}, Basilio and {Sayres}, Conor and {Schiavon}, Ricardo and {Schlegel}, David J. and {Schlesinger}, Katharine J. and {Schmidt}, Sarah J. and {Schneider}, Donald P. and {Sellgren}, Kris and {Shelden}, Alaina and {Sheldon}, Erin and {Shetrone}, Matthew and {Shu}, Yiping and {Silverman}, John D. and {Simmerer}, Jennifer and {Simmons}, Audrey E. and {Sivarani}, Thirupathi and {Skrutskie}, M.~F. and {Slosar}, An{\v{z}}e and {Smee}, Stephen and {Smith}, Verne V. and {Snedden}, Stephanie A. and {Stassun}, Keivan G. and {Steele}, Oliver and {Steinmetz}, Matthias and {Stockett}, Mark H. and {Stollberg}, Todd and {Strauss}, Michael A. and {Szalay}, Alexander S. and {Tanaka}, Masayuki and {Thakar}, Aniruddha R. and {Thomas}, Daniel and {Tinker}, Jeremy L. and {Tofflemire}, Benjamin M. and {Tojeiro}, Rita and {Tremonti}, Christy A. and {Vargas Maga{\~n}a}, Mariana and {Verde}, Licia and {Vogt}, Nicole P. and {Wake}, David A. and {Wan}, Xiaoke and {Wang}, Ji and {Weaver}, Benjamin A. and {White}, Martin and {White}, Simon D.~M. and {Wilson}, John C. and {Wisniewski}, John P. and {Wood-Vasey}, W. Michael and {Yanny}, Brian and {Yasuda}, Naoki and {Y{\`e}che}, Christophe and {York}, Donald G. and {Young}, Erick and {Zasowski}, Gail and {Zehavi}, Idit and {Zhao}, Bo},
        title = "{SDSS-III: Massive Spectroscopic Surveys of the Distant Universe, the Milky Way, and Extra-Solar Planetary Systems}",
      journal = {\aj},
     keywords = {cosmology: observations, Galaxy: evolution, planets and satellites: detection, surveys, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2011,
        month = sep,
       volume = {142},
       number = {3},
          eid = {72},
        pages = {72},
          doi = {10.1088/0004-6256/142/3/72},
archivePrefix = {arXiv},
       eprint = {1101.1529},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011AJ....142...72E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{BOSSDR1112,
       author = {{Alam}, Shadab and {Albareti}, Franco D. and {Allende Prieto}, Carlos and {Anders}, F. and {Anderson}, Scott F. and {Anderton}, Timothy and {Andrews}, Brett H. and {Armengaud}, Eric and {Aubourg}, {\'E}ric and {Bailey}, Stephen and {Basu}, Sarbani and {Bautista}, Julian E. and {Beaton}, Rachael L. and {Beers}, Timothy C. and {Bender}, Chad F. and {Berlind}, Andreas A. and {Beutler}, Florian and {Bhardwaj}, Vaishali and {Bird}, Jonathan C. and {Bizyaev}, Dmitry and {Blake}, Cullen H. and {Blanton}, Michael R. and {Blomqvist}, Michael and {Bochanski}, John J. and {Bolton}, Adam S. and {Bovy}, Jo and {Shelden Bradley}, A. and {Brandt}, W.~N. and {Brauer}, D.~E. and {Brinkmann}, J. and {Brown}, Peter J. and {Brownstein}, Joel R. and {Burden}, Angela and {Burtin}, Etienne and {Busca}, Nicol{\'a}s G. and {Cai}, Zheng and {Capozzi}, Diego and {Carnero Rosell}, Aurelio and {Carr}, Michael A. and {Carrera}, Ricardo and {Chambers}, K.~C. and {Chaplin}, William James and {Chen}, Yen-Chi and {Chiappini}, Cristina and {Chojnowski}, S. Drew and {Chuang}, Chia-Hsun and {Clerc}, Nicolas and {Comparat}, Johan and {Covey}, Kevin and {Croft}, Rupert A.~C. and {Cuesta}, Antonio J. and {Cunha}, Katia and {da Costa}, Luiz N. and {Da Rio}, Nicola and {Davenport}, James R.~A. and {Dawson}, Kyle S. and {De Lee}, Nathan and {Delubac}, Timoth{\'e}e and {Deshpande}, Rohit and {Dhital}, Saurav and {Dutra-Ferreira}, Let{\'\i}cia and {Dwelly}, Tom and {Ealet}, Anne and {Ebelke}, Garrett L. and {Edmondson}, Edward M. and {Eisenstein}, Daniel J. and {Ellsworth}, Tristan and {Elsworth}, Yvonne and {Epstein}, Courtney R. and {Eracleous}, Michael and {Escoffier}, Stephanie and {Esposito}, Massimiliano and {Evans}, Michael L. and {Fan}, Xiaohui and {Fern{\'a}ndez-Alvar}, Emma and {Feuillet}, Diane and {Filiz Ak}, Nurten and {Finley}, Hayley and {Finoguenov}, Alexis and {Flaherty}, Kevin and {Fleming}, Scott W. and {Font-Ribera}, Andreu and {Foster}, Jonathan and {Frinchaboy}, Peter M. and {Galbraith-Frew}, J.~G. and {Garc{\'\i}a}, Rafael A. and {Garc{\'\i}a-Hern{\'a}ndez}, D.~A. and {Garc{\'\i}a P{\'e}rez}, Ana E. and {Gaulme}, Patrick and {Ge}, Jian and {G{\'e}nova-Santos}, R. and {Georgakakis}, A. and {Ghezzi}, Luan and {Gillespie}, Bruce A. and {Girardi}, L{\'e}o and {Goddard}, Daniel and {Gontcho}, Satya Gontcho A. and {Gonz{\'a}lez Hern{\'a}ndez}, Jonay I. and {Grebel}, Eva K. and {Green}, Paul J. and {Grieb}, Jan Niklas and {Grieves}, Nolan and {Gunn}, James E. and {Guo}, Hong and {Harding}, Paul and {Hasselquist}, Sten and {Hawley}, Suzanne L. and {Hayden}, Michael and {Hearty}, Fred R. and {Hekker}, Saskia and {Ho}, Shirley and {Hogg}, David W. and {Holley-Bockelmann}, Kelly and {Holtzman}, Jon A. and {Honscheid}, Klaus and {Huber}, Daniel and {Huehnerhoff}, Joseph and {Ivans}, Inese I. and {Jiang}, Linhua and {Johnson}, Jennifer A. and {Kinemuchi}, Karen and {Kirkby}, David and {Kitaura}, Francisco and {Klaene}, Mark A. and {Knapp}, Gillian R. and {Kneib}, Jean-Paul and {Koenig}, Xavier P. and {Lam}, Charles R. and {Lan}, Ting-Wen and {Lang}, Dustin and {Laurent}, Pierre and {Le Goff}, Jean-Marc and {Leauthaud}, Alexie and {Lee}, Khee-Gan and {Lee}, Young Sun and {Licquia}, Timothy C. and {Liu}, Jian and {Long}, Daniel C. and {L{\'o}pez-Corredoira}, Mart{\'\i}n and {Lorenzo-Oliveira}, Diego and {Lucatello}, Sara and {Lundgren}, Britt and {Lupton}, Robert H. and {Mack}, Claude E., III and {Mahadevan}, Suvrath and {Maia}, Marcio A.~G. and {Majewski}, Steven R. and {Malanushenko}, Elena and {Malanushenko}, Viktor and {Manchado}, A. and {Manera}, Marc and {Mao}, Qingqing and {Maraston}, Claudia and {Marchwinski}, Robert C. and {Margala}, Daniel and {Martell}, Sarah L. and {Martig}, Marie and {Masters}, Karen L. and {Mathur}, Savita and {McBride}, Cameron K. and {McGehee}, Peregrine M. and {McGreer}, Ian D. and {McMahon}, Richard G. and {M{\'e}nard}, Brice and {Menzel}, Marie-Luise and {Merloni}, Andrea and {M{\'e}sz{\'a}ros}, Szabolcs and {Miller}, Adam A. and {Miralda-Escud{\'e}}, Jordi and {Miyatake}, Hironao and {Montero-Dorta}, Antonio D. and {More}, Surhud and {Morganson}, Eric and {Morice-Atkinson}, Xan and {Morrison}, Heather L. and {Mosser}, Ben{\^o}it and {Muna}, Demitri and {Myers}, Adam D. and {Nandra}, Kirpal and {Newman}, Jeffrey A. and {Neyrinck}, Mark and {Nguyen}, Duy Cuong and {Nichol}, Robert C. and {Nidever}, David L. and {Noterdaeme}, Pasquier and {Nuza}, Sebasti{\'a}n E. and {O'Connell}, Julia E. and {O'Connell}, Robert W. and {O'Connell}, Ross and {Ogando}, Ricardo L.~C. and {Olmstead}, Matthew D. and {Oravetz}, Audrey E. and {Oravetz}, Daniel J. and {Osumi}, Keisuke and {Owen}, Russell and {Padgett}, Deborah L. and {Padmanabhan}, Nikhil and {Paegert}, Martin and {Palanque-Delabrouille}, Nathalie and {Pan}, Kaike and {Parejko}, John K. and {P{\^a}ris}, Isabelle and {Park}, Changbom and {Pattarakijwanich}, Petchara and {Pellejero-Ibanez}, M. and {Pepper}, Joshua and {Percival}, Will J. and {P{\'e}rez-Fournon}, Ismael and {P{\'e}rez-R{\`a}fols}, Ignasi and {Petitjean}, Patrick and {Pieri}, Matthew M. and {Pinsonneault}, Marc H. and {Porto de Mello}, Gustavo F. and {Prada}, Francisco and {Prakash}, Abhishek and {Price-Whelan}, Adrian M. and {Protopapas}, Pavlos and {Raddick}, M. Jordan and {Rahman}, Mubdi and {Reid}, Beth A. and {Rich}, James and {Rix}, Hans-Walter and {Robin}, Annie C. and {Rockosi}, Constance M. and {Rodrigues}, Tha{\'\i}se S. and {Rodr{\'\i}guez-Torres}, Sergio and {Roe}, Natalie A. and {Ross}, Ashley J. and {Ross}, Nicholas P. and {Rossi}, Graziano and {Ruan}, John J. and {Rubi{\~n}o-Mart{\'\i}n}, J.~A. and {Rykoff}, Eli S. and {Salazar-Albornoz}, Salvador and {Salvato}, Mara and {Samushia}, Lado and {S{\'a}nchez}, Ariel G. and {Santiago}, Bas{\'\i}lio and {Sayres}, Conor and {Schiavon}, Ricardo P. and {Schlegel}, David J. and {Schmidt}, Sarah J. and {Schneider}, Donald P. and {Schultheis}, Mathias and {Schwope}, Axel D. and {Sc{\'o}ccola}, C.~G. and {Scott}, Caroline and {Sellgren}, Kris and {Seo}, Hee-Jong and {Serenelli}, Aldo and {Shane}, Neville and {Shen}, Yue and {Shetrone}, Matthew and {Shu}, Yiping and {Silva Aguirre}, V. and {Sivarani}, Thirupathi and {Skrutskie}, M.~F. and {Slosar}, An{\v{z}}e and {Smith}, Verne V. and {Sobreira}, Fl{\'a}via and {Souto}, Diogo and {Stassun}, Keivan G. and {Steinmetz}, Matthias and {Stello}, Dennis and {Strauss}, Michael A. and {Streblyanska}, Alina and {Suzuki}, Nao and {Swanson}, Molly E.~C. and {Tan}, Jonathan C. and {Tayar}, Jamie and {Terrien}, Ryan C. and {Thakar}, Aniruddha R. and {Thomas}, Daniel and {Thomas}, Neil and {Thompson}, Benjamin A. and {Tinker}, Jeremy L. and {Tojeiro}, Rita and {Troup}, Nicholas W. and {Vargas-Maga{\~n}a}, Mariana and {Vazquez}, Jose A. and {Verde}, Licia and {Viel}, Matteo and {Vogt}, Nicole P. and {Wake}, David A. and {Wang}, Ji and {Weaver}, Benjamin A. and {Weinberg}, David H. and {Weiner}, Benjamin J. and {White}, Martin and {Wilson}, John C. and {Wisniewski}, John P. and {Wood-Vasey}, W.~M. and {Ye`che}, Christophe and {York}, Donald G. and {Zakamska}, Nadia L. and {Zamora}, O. and {Zasowski}, Gail and {Zehavi}, Idit and {Zhao}, Gong-Bo and {Zheng}, Zheng and {Zhou}, Xu and {Zhou}, Zhimin and {Zou}, Hu and {Zhu}, Guangtun},
        title = "{The Eleventh and Twelfth Data Releases of the Sloan Digital Sky Survey: Final Data from SDSS-III}",
      journal = {\apjs},
     keywords = {atlases, catalogs, surveys, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = jul,
       volume = {219},
       number = {1},
          eid = {12},
        pages = {12},
          doi = {10.1088/0067-0049/219/1/12},
archivePrefix = {arXiv},
       eprint = {1501.00963},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJS..219...12A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{GrowthIndex,
       author = {{Linder}, Eric V. and {Cahn}, Robert N.},
        title = "{Parameterized beyond-Einstein growth}",
      journal = {Astroparticle Physics},
     keywords = {Cosmology, Dark energy, Astrophysics, General Relativity and Quantum Cosmology},
         year = 2007,
        month = dec,
       volume = {28},
       number = {4-5},
        pages = {481-488},
          doi = {10.1016/j.astropartphys.2007.09.003},
archivePrefix = {arXiv},
       eprint = {astro-ph/0701317},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007APh....28..481L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{RSDScoccimarro,
       author = {{Scoccimarro}, Rom{\'a}n},
        title = "{Redshift-space distortions, pairwise velocities, and nonlinearities}",
      journal = {\prd},
     keywords = {98.62.Py, 98.65.Dx, Distances redshifts radial velocities, spatial distribution of galaxies, Superclusters, large-scale structure of the Universe, Astrophysics},
         year = 2004,
        month = oct,
       volume = {70},
       number = {8},
          eid = {083007},
        pages = {083007},
          doi = {10.1103/PhysRevD.70.083007},
archivePrefix = {arXiv},
       eprint = {astro-ph/0407214},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004PhRvD..70h3007S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{RSDKaiser,
       author = {{Kaiser}, Nick},
        title = "{Clustering in real space and in redshift space}",
      journal = {\mnras},
     keywords = {Astronomical Models, Deep Space, Galactic Clusters, Red Shift, Density Distribution, Power Spectra, Velocity Distribution, Astrophysics},
         year = 1987,
        month = jul,
       volume = {227},
        pages = {1-21},
          doi = {10.1093/mnras/227.1.1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1987MNRAS.227....1K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{NonLinear1,
       author = {{Davis}, M. and {Peebles}, P.~J.~E.},
        title = "{A survey of galaxy redshifts. V. The two-point position and velocity correlations.}",
      journal = {\apj},
     keywords = {Cosmology, Galactic Clusters, Galaxies, Red Shift, Correlation, Line Of Sight, Mass Distribution, Position (Location), Velocity Distribution, Astrophysics},
         year = 1983,
        month = apr,
       volume = {267},
        pages = {465-482},
          doi = {10.1086/160884},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1983ApJ...267..465D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{NonLinear2,
       author = {{Kaiser}, Nick},
        title = "{Clustering in real space and in redshift space}",
      journal = {\mnras},
     keywords = {Astronomical Models, Deep Space, Galactic Clusters, Red Shift, Density Distribution, Power Spectra, Velocity Distribution, Astrophysics},
         year = 1987,
        month = jul,
       volume = {227},
        pages = {1-21},
          doi = {10.1093/mnras/227.1.1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1987MNRAS.227....1K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{MiniJPAS,
	doi = {10.1051/0004-6361/202038841},
  
	url = {https://doi.org/10.1051%2F0004-6361%2F202038841},
  
	year = 2021,
	month = {sep},
  
	publisher = {{EDP} Sciences},
  
	volume = {653},
  
	pages = {A31},
  
	author = {S. Bonoli and A. Mar{\'{\i}
}n-Franch and J. Varela and H. V{\'{a}}zquez Rami{\'{o}} and L. R. Abramo and A. J. Cenarro and R. A. Dupke and J. M. V{\'{\i}}lchez and D. Crist{\'{o}}bal-Hornillos and R. M. Gonz{\'{a}}lez Delgado and C. Hern{\'{a}}ndez-Monteagudo and C. L{\'{o}}pez-Sanjuan and D. J. Muniesa and T. Civera and A. Ederoclite and A. Hern{\'{a}}n-Caballero and V. Marra and P. O. Baqui and A. Cortesi and E. S. Cypriano and S. Daflon and A. L. de Amorim and L. A. D{\'{\i}}az-Garc{\'{\i}}a and J. M. Diego and G. Mart{\'{\i}}nez-Solaeche and E. P{\'{e}}rez and V. M. Placco and F. Prada and C. Queiroz and J. Alcaniz and A. Alvarez-Candal and J. Cepa and A. L. Maroto and F. Roig and B. B. Siffert and K. Taylor and N. Benitez and M. Moles and L. Sodr{\'{e}} and S. Carneiro and C. Mendes de Oliveira and E. Abdalla and R. E. Angulo and M. Aparicio Resco and A. Balaguera-Antol{\'{\i}}nez and F. J. Ballesteros and D. Brito-Silva and T. Broadhurst and E. R. Carrasco and T. Castro and R. Cid Fernandes and P. Coelho and R. B. de Melo and L. Doubrawa and A. Fernandez-Soto and F. Ferrari and A. Finoguenov and R. Garc{\'{\i}}a-Benito and J. Iglesias-P{\'{a}}ramo and Y. Jim{\'{e}}nez-Teja and F. S. Kitaura and J. Laur and P. A. A. Lopes and G. Lucatelli and V. J. Mart{\'{\i}}nez and M. Maturi and R. A. Overzier and C. Pigozzo and M. Quartin and J. E. Rodr{\'{\i}}guez-Mart{\'{\i}}n and V. Salzano and A. Tamm and E. Tempel and K. Umetsu and L. Valdivielso and R. von Marttens and A. Zitrin and M. C. D{\'{\i}}az-Mart{\'{\i}}n and G. L{\'{o}}pez-Alegre and A. L{\'{o}}pez-Sainz and A. Yanes-D{\'{\i}}az and F. Rueda-Teruel and S. Rueda-Teruel and J. Abril Iba{\~{n}}ez and J. L Ant{\'{o}}n Bravo and R. Bello Ferrer and S. Bielsa and J. M. Casino and J. Castillo and S. Chueca and L. Cuesta and J. Garzar{\'{a}}n Calderaro and R. Iglesias-Marzoa and C. {\'{I}}niguez and J. L. Lamadrid Gutierrez and F. Lopez-Martinez and D. Lozano-P{\'{e}}rez and N. Ma{\'{\i}}cas Sacrist{\'{a}}n and E. L. Molina-Ib{\'{a}}{\~{n}}ez and A. Moreno-Signes and S. Rodr{\'{\i}}guez Llano and M. Royo Navarro and V. Tilve Rua and U. Andrade and E. J. Alfaro and S. Akras and P. Arnalte-Mur and B. Ascaso and C. E. Barbosa and J. Beltr{\'{a}}n Jim{\'{e}}nez and M. Benetti and C. A. P. Bengaly and A. Bernui and J. J. Blanco-Pillado and M. Borges Fernandes and J. N. Bregman and G. Bruzual and G. Calderone and J. M. Carvano and L. Casarini and J. Chaves-Montero and A. L. Chies-Santos and G. Coutinho de Carvalho and P. Dimauro and S. Duarte Puertas and D. Figueruelo and J. I. Gonz{\'{a}}lez-Serrano and M. A. Guerrero and S. Gurung-L{\'{o}}pez and D. Herranz and M. Huertas-Company and J. A. Irwin and D. Izquierdo-Villalba and A. Kanaan and C. Kehrig and C. C. Kirkpatrick and J. Lim and A. R. Lopes and R. Lopes de Oliveira and A. Marcos-Caballero and D. Mart{\'{\i}}nez-Delgado and E. Mart{\'{\i}}nez-Gonz{\'{a}}lez and G. Mart{\'{\i}}nez-Somonte and N. Oliveira and A. A. Orsi and M. Penna-Lima and R. R. R. Reis and D. Spinoso and S. Tsujikawa and P. Vielva and A. Z. Vitorelli and J. Q. Xia and H. B. Yuan and A. Arroyo-Polonio and M. L. L. Dantas and C. A. Galarza and D. R. Gon{\c{c}}alves and R. S. Gon{\c{c}}alves and J. E. Gonzalez and A. H. Gonzalez and N. Greisel and F. Jim{\'{e}}nez-Esteban and R. G. Landim and D. Lazzaro and G. Magris and R. Monteiro-Oliveira and C. B. Pereira and M. J. Rebou{\c{c}}as and J. M. Rodriguez-Espinosa and S. Santos da Costa and E. Telles},
  
	title = {The {miniJPAS} survey: A preview of the Universe in 56 colors},
  
	journal = {Astronomy {\&}amp$\mathsemicolon$ Astrophysics}
}


@ARTICLE{WMAPAnomalies,
       author = {{Bennett}, C.~L. and {Hill}, R.~S. and {Hinshaw}, G. and {Larson}, D. and {Smith}, K.~M. and {Dunkley}, J. and {Gold}, B. and {Halpern}, M. and {Jarosik}, N. and {Kogut}, A. and {Komatsu}, E. and {Limon}, M. and {Meyer}, S.~S. and {Nolta}, M.~R. and {Odegard}, N. and {Page}, L. and {Spergel}, D.~N. and {Tucker}, G.~S. and {Weiland}, J.~L. and {Wollack}, E. and {Wright}, E.~L.},
        title = "{Seven-year Wilkinson Microwave Anisotropy Probe (WMAP) Observations: Are There Cosmic Microwave Background Anomalies?}",
      journal = {\apjs},
     keywords = {cosmic background radiation, cosmological parameters, cosmology: observations, dark matter, early universe, instrumentation: detectors, large-scale structure of universe, space vehicles, space vehicles: instruments, telescopes, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2011,
        month = feb,
       volume = {192},
       number = {2},
          eid = {17},
        pages = {17},
          doi = {10.1088/0067-0049/192/2/17},
archivePrefix = {arXiv},
       eprint = {1001.4758},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJS..192...17B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{QueirozQSOMocks,
       author = {{Queiroz}, Carolina and {Abramo}, L. Raul and {Rodrigues}, Nat{\'a}lia V.~N. and {P{\'e}rez-R{\`a}fols}, Ignasi and {Mart{\'\i}nez-Solaeche}, Gin{\'e}s and {Hern{\'a}n-Caballero}, Antonio and {Hern{\'a}ndez-Monteagudo}, Carlos and {Lumbreras-Calle}, Alejandro and {Pieri}, Matthew M. and {Morrison}, Sean S. and {Bonoli}, Silvia and {Chaves-Montero}, Jon{\'a}s and {Chies-Santos}, Ana L. and {D{\'\i}az-Garc{\'\i}a}, L.~A. and {Fernandez-Soto}, Alberto and {Gonz{\'a}lez Delgado}, Rosa M. and {Alcaniz}, Jailson and {Ben{\'\i}tez}, Narciso and {Cenarro}, A. Javier and {Civera}, Tamara and {Dupke}, Renato A. and {Ederoclite}, Alessandro and {L{\'o}pez-Sanjuan}, Carlos and {Mar{\'\i}n-Franch}, Antonio and {Mendes de Oliveira}, Claudia and {Moles}, Mariano and {Muniesa}, David and {Sodr{\'e}}, Laerte and {Taylor}, Keith and {Varela}, Jes{\'u}s and {V{\'a}zquez Rami{\'o}}, H{\'e}ctor},
        title = "{The miniJPAS survey quasar selection I: Mock catalogues for classification}",
      journal = {\mnras},
     keywords = {quasars: general, methods: data analysis, surveys, catalogues, techniques: photometric, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2022,
        month = oct,
          doi = {10.1093/mnras/stac2962},
archivePrefix = {arXiv},
       eprint = {2202.00103},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.tmp.2757Q},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@unpublished{QueirozPreparation,
      author = {{Queiroz et al.}, Carolina},
        title = {In preparation},
         year = {(2023)},
      note = {Unpublished}
}

@ARTICLE{ReconLinearInterpolation1,
       author = {{Hannestad}, Steen},
        title = "{Reconstructing the primordial power spectrum{\textemdash}a new algorithm}",
      journal = {\jcap},
     keywords = {Astrophysics, High Energy Physics - Phenomenology},
         year = 2004,
        month = apr,
       volume = {2004},
       number = {4},
          eid = {002},
        pages = {002},
          doi = {10.1088/1475-7516/2004/04/002},
archivePrefix = {arXiv},
       eprint = {astro-ph/0311491},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004JCAP...04..002H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ReconBridle,
       author = {{Bridle}, S.~L. and {Lewis}, A.~M. and {Weller}, J. and {Efstathiou}, G.},
        title = "{Reconstructing the primordial power spectrum}",
      journal = {\mnras},
     keywords = {cosmic microwave background, cosmology: observations, cosmology: theory, large-scale structure of Universe, Astrophysics, High Energy Physics - Phenomenology},
         year = 2003,
        month = jul,
       volume = {342},
       number = {4},
        pages = {L72-L78},
          doi = {10.1046/j.1365-8711.2003.06807.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0302306},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003MNRAS.342L..72B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Parametric1Contaldi2003,
       author = {{Contaldi}, Carlo R. and {Peloso}, Marco and {Kofman}, Lev and {Linde}, Andrei},
        title = "{Suppressing the lower multipoles in the CMB anisotropies}",
      journal = {\jcap},
     keywords = {Astrophysics, General Relativity and Quantum Cosmology, High Energy Physics - Phenomenology, High Energy Physics - Theory},
         year = 2003,
        month = jul,
       volume = {2003},
       number = {7},
          eid = {002},
        pages = {002},
          doi = {10.1088/1475-7516/2003/07/002},
archivePrefix = {arXiv},
       eprint = {astro-ph/0303636},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003JCAP...07..002C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Parametric2Sinha2006,
       author = {{Sinha}, Rita and {Souradeep}, Tarun},
        title = "{Post-WMAP assessment of infrared cutoff in the primordial spectrum from inflation}",
      journal = {\prd},
     keywords = {98.80.Cq, 98.80.-k, Particle-theory and field-theory models of the early Universe, Cosmology, Astrophysics},
         year = 2006,
        month = aug,
       volume = {74},
       number = {4},
          eid = {043518},
        pages = {043518},
          doi = {10.1103/PhysRevD.74.043518},
archivePrefix = {arXiv},
       eprint = {astro-ph/0511808},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006PhRvD..74d3518S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Parametric3Simon2005,
       author = {{Simon}, Joan and {Verde}, Licia and {Jimenez}, Raul},
        title = "{Constraints on the redshift dependence of the dark energy potential}",
      journal = {\prd},
     keywords = {98.62.Py, 98.80.Cq, Distances redshifts radial velocities, spatial distribution of galaxies, Particle-theory and field-theory models of the early Universe, Astrophysics, High Energy Physics - Theory},
         year = 2005,
        month = jun,
       volume = {71},
       number = {12},
          eid = {123001},
        pages = {123001},
          doi = {10.1103/PhysRevD.71.123001},
archivePrefix = {arXiv},
       eprint = {astro-ph/0412269},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005PhRvD..71l3001S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Parametric4Bridges2006,
       author = {{Bridges}, M. and {Lasenby}, A.~N. and {Hobson}, M.~P.},
        title = "{A Bayesian analysis of the primordial power spectrum}",
      journal = {\mnras},
     keywords = {cosmic microwave background: cosmological parameters: cosmology: observations: cosmology: theory: large-scale structure of Universe, cosmic microwave background, cosmological parameters, cosmology: observations, cosmology: theory, large-scale structure of Universe, Astrophysics},
         year = 2006,
        month = jul,
       volume = {369},
       number = {3},
        pages = {1123-1130},
          doi = {10.1111/j.1365-2966.2006.10351.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0511573},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006MNRAS.369.1123B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Parametric5Bridges2007,
       author = {{Bridges}, M. and {Lasenby}, A.~N. and {Hobson}, M.~P.},
        title = "{WMAP 3-yr primordial power spectrum}",
      journal = {\mnras},
     keywords = {cosmic microwave background, cosmological parameters, cosmology: observations, cosmology: theory, large-scale structure of Universe, Astrophysics},
         year = 2007,
        month = oct,
       volume = {381},
       number = {1},
        pages = {68-74},
          doi = {10.1111/j.1365-2966.2007.11778.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0607404},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007MNRAS.381...68B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Parametric6Covi2006,
       author = {{Covi}, Laura and {Hamann}, Jan and {Melchiorri}, Alessandro and {Slosar}, An{\v{z}}e and {Sorbera}, Irene},
        title = "{Inflation and WMAP three year data: Features are still present}",
      journal = {\prd},
     keywords = {98.80.Cq, Particle-theory and field-theory models of the early Universe, Astrophysics},
         year = 2006,
        month = oct,
       volume = {74},
       number = {8},
          eid = {083509},
        pages = {083509},
          doi = {10.1103/PhysRevD.74.083509},
archivePrefix = {arXiv},
       eprint = {astro-ph/0606452},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006PhRvD..74h3509C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Parametric7Joy2009,
       author = {{Joy}, Minu and {Shafieloo}, Arman and {Sahni}, Varun and {Starobinsky}, Alexei A.},
        title = "{Is a step in the primordial spectral index favoured by CMB data?}",
      journal = {\jcap},
     keywords = {Astrophysics, General Relativity and Quantum Cosmology, High Energy Physics - Theory},
         year = 2009,
        month = jun,
       volume = {2009},
       number = {6},
          eid = {028},
        pages = {028},
          doi = {10.1088/1475-7516/2009/06/028},
archivePrefix = {arXiv},
       eprint = {0807.3334},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009JCAP...06..028J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Parametric8Paykari2010,
       author = {{Paykari}, Paniez and {Jaffe}, Andrew H.},
        title = "{Optimal Binning of the Primordial Power Spectrum}",
      journal = {\apj},
     keywords = {cosmic background radiation, cosmological parameters, early universe, large-scale structure of universe, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2010,
        month = mar,
       volume = {711},
       number = {1},
        pages = {1-12},
          doi = {10.1088/0004-637X/711/1/1},
archivePrefix = {arXiv},
       eprint = {0902.4399},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...711....1P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Parametric9Guo2011,
       author = {{Guo}, Zong-Kuan and {Schwarz}, Dominik J. and {Zhang}, Yuan-Zhong},
        title = "{Reconstruction of the primordial power spectrum from CMB data}",
      journal = {\jcap},
     keywords = {Astrophysics - Cosmology and Extragalactic Astrophysics, General Relativity and Quantum Cosmology, High Energy Physics - Phenomenology, High Energy Physics - Theory},
         year = 2011,
        month = aug,
       volume = {2011},
       number = {8},
          eid = {031},
        pages = {031},
          doi = {10.1088/1475-7516/2011/08/031},
archivePrefix = {arXiv},
       eprint = {1105.5916},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011JCAP...08..031G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Parametric10Goswami2013,
       author = {{Goswami}, Gaurav and {Prasad}, Jayanti},
        title = "{Maximum entropy deconvolution of primordial power spectrum}",
      journal = {\prd},
     keywords = {98.80.Es, 98.70.Vc, Observational cosmology, Background radiations, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2013,
        month = jul,
       volume = {88},
       number = {2},
          eid = {023522},
        pages = {023522},
          doi = {10.1103/PhysRevD.88.023522},
archivePrefix = {arXiv},
       eprint = {1303.4747},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013PhRvD..88b3522G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ChlubaFeatures,
       author = {{Chluba}, Jens and {Hamann}, Jan and {Patil}, Subodh P.},
        title = "{Features and new physical scales in primordial observables: Theory and observation}",
      journal = {International Journal of Modern Physics D},
     keywords = {Cosmology, inflation, 98.80.-k, 98.80.Cq, Cosmology, Particle-theory and field-theory models of the early Universe, Astrophysics - Cosmology and Nongalactic Astrophysics, High Energy Physics - Phenomenology, High Energy Physics - Theory},
         year = 2015,
        month = jun,
       volume = {24},
       number = {10},
          eid = {1530023},
        pages = {1530023},
          doi = {10.1142/S0218271815300232},
archivePrefix = {arXiv},
       eprint = {1505.01834},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015IJMPD..2430023C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{FoGPaper,
       author = {{Percival}, Will J. and {Burkey}, Daniel and {Heavens}, Alan and {Taylor}, Andy and {Cole}, Shaun and {Peacock}, John A. and {Baugh}, Carlton M. and {Bland-Hawthorn}, Joss and {Bridges}, Terry and {Cannon}, Russell and {Colless}, Matthew and {Collins}, Chris and {Couch}, Warrick and {Dalton}, Gavin and {De Propris}, Roberto and {Driver}, Simon P. and {Efstathiou}, George and {Ellis}, Richard S. and {Frenk}, Carlos S. and {Glazebrook}, Karl and {Jackson}, Carole and {Lahav}, Ofer and {Lewis}, Ian and {Lumsden}, Stuart and {Maddox}, Steve and {Norberg}, Peder and {Peterson}, Bruce A. and {Sutherland}, Will and {Taylor}, Keith},
        title = "{The 2dF Galaxy Redshift Survey: spherical harmonics analysis of fluctuations in the final catalogue}",
      journal = {\mnras},
     keywords = {cosmological parameters, large-scale structure of Universe, Astrophysics},
         year = 2004,
        month = oct,
       volume = {353},
       number = {4},
        pages = {1201-1218},
          doi = {10.1111/j.1365-2966.2004.08146.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0406513},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004MNRAS.353.1201P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{APEffectOriginal,
       author = {{Alcock}, C. and {Paczynski}, B.},
        title = "{An evolution free test for non-zero cosmological constant}",
      journal = {\nat},
     keywords = {Astrophysics},
         year = 1979,
        month = oct,
       volume = {281},
        pages = {358},
          doi = {10.1038/281358a0},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1979Natur.281..358A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{AgnosticBOSS,
       author = {{Brieden}, Samuel and {Gil-Mar{\'\i}n}, H{\'e}ctor and {Verde}, Licia},
        title = "{Model-agnostic interpretation of 10 billion years of cosmic evolution traced by BOSS and eBOSS data}",
      journal = {\jcap},
     keywords = {baryon acoustic oscillations, cosmological parameters from LSS, galaxy surveys, power spectrum, Astrophysics - Cosmology and Nongalactic Astrophysics, General Relativity and Quantum Cosmology},
         year = 2022,
        month = aug,
       volume = {2022},
       number = {8},
          eid = {024},
        pages = {024},
          doi = {10.1088/1475-7516/2022/08/024},
archivePrefix = {arXiv},
       eprint = {2204.11868},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022JCAP...08..024B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{EuclidForecastModel,
       author = {{Casas}, S. and {Lesgourgues}, J. and {Sch{\"o}neberg}, N. and {Sabarish V.}, M. and {Rathmann}, L. and {Doerenkamp}, M. and {Archidiacono}, M. and {Bellini}, E. and {Clesse}, S. and {Frusciante}, N. and {Martinelli}, M. and {Pace}, F. and {Sapone}, D. and {Sakr}, Z. and {Blanchard}, A. and {Brinckmann}, T. and {Camera}, S. and {Carbone}, C. and {Ili{\'c}}, S. and {Markovic}, K. and {Pettorino}, V. and {Tutusaus}, I. and {Aghanim}, N. and {Amara}, A. and {Amendola}, L. and {Auricchio}, N. and {Baldi}, M. and {Bonino}, D. and {Branchini}, E. and {Brescia}, M. and {Brinchmann}, J. and {Capobianco}, V. and {Cardone}, V.~F. and {Carretero}, J. and {Castellano}, M. and {Cavuoti}, S. and {Cimatti}, A. and {Cledassou}, R. and {Congedo}, G. and {Conversi}, L. and {Copin}, Y. and {Corcione}, L. and {Courbin}, F. and {Cropper}, M. and {Degaudenzi}, H. and {Dinis}, J. and {Douspis}, M. and {Dubath}, F. and {Dupac}, X. and {Dusini}, S. and {Farrens}, S. and {Frailis}, M. and {Franceschi}, E. and {Fumana}, M. and {Galeotta}, S. and {Garilli}, B. and {Gillis}, B. and {Giocoli}, C. and {Grazian}, A. and {Grupp}, F. and {Haugan}, S.~V.~H. and {Hormuth}, F. and {Hornstrup}, A. and {Jahnke}, K. and {K{\"u}mmel}, M. and {Kiessling}, A. and {Kilbinger}, M. and {Kitching}, T. and {Kunz}, M. and {Kurki-Suonio}, H. and {Ligori}, S. and {Lilje}, P.~B. and {Lloro}, I. and {Mansutti}, O. and {Marggraf}, O. and {Marulli}, F. and {Massey}, R. and {Medinaceli}, E. and {Mei}, S. and {Meneghetti}, M. and {Merlin}, E. and {Meylan}, G. and {Moresco}, M. and {Moscardini}, L. and {Munari}, E. and {Niemi}, S. -M. and {Padilla}, C. and {Paltani}, S. and {Pasian}, F. and {Pedersen}, K. and {Percival}, W.~J. and {Pires}, S. and {Polenta}, G. and {Poncet}, M. and {Popa}, L.~A. and {Raison}, F. and {Renzi}, A. and {Rhodes}, J. and {Riccio}, G. and {Romelli}, E. and {Roncarelli}, M. and {Rossetti}, E. and {Saglia}, R. and {Sartoris}, B. and {Schneider}, P. and {Secroun}, A. and {Seidel}, G. and {Serrano}, S. and {Sirignano}, C. and {Sirri}, G. and {Stanco}, L. and {Starck}, J. -L. and {Surace}, C. and {Tallada-Cresp{\'\i}}, P. and {Taylor}, A.~N. and {Tereno}, I. and {Toledo-Moreo}, R. and {Torradeflot}, F. and {Valentijn}, E.~A. and {Valenziano}, L. and {Vassallo}, T. and {Wang}, Y. and {Weller}, J. and {Zamorani}, G. and {Zoubian}, J. and {Scottez}, V. and {Veropalumbo}, A.},
        title = "{Euclid: Validation of the MontePython forecasting tools}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2023,
        month = mar,
          eid = {arXiv:2303.09451},
        pages = {arXiv:2303.09451},
          doi = {10.48550/arXiv.2303.09451},
archivePrefix = {arXiv},
       eprint = {2303.09451},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023arXiv230309451C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Beutler2014,
       author = {{Beutler}, Florian and {Saito}, Shun and {Seo}, Hee-Jong and {Brinkmann}, Jon and {Dawson}, Kyle S. and {Eisenstein}, Daniel J. and {Font-Ribera}, Andreu and {Ho}, Shirley and {McBride}, Cameron K. and {Montesano}, Francesco and {Percival}, Will J. and {Ross}, Ashley J. and {Ross}, Nicholas P. and {Samushia}, Lado and {Schlegel}, David J. and {S{\'a}nchez}, Ariel G. and {Tinker}, Jeremy L. and {Weaver}, Benjamin A.},
        title = "{The clustering of galaxies in the SDSS-III Baryon Oscillation Spectroscopic Survey: testing gravity with redshift space distortions using the power spectrum multipoles}",
      journal = {\mnras},
     keywords = {gravitation, surveys, cosmological parameters, cosmology: observations, dark energy, large-scale structure of Universe, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2014,
        month = sep,
       volume = {443},
       number = {2},
        pages = {1065-1089},
          doi = {10.1093/mnras/stu1051},
archivePrefix = {arXiv},
       eprint = {1312.4611},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.443.1065B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{GilMarin2015a,
       author = {{Gil-Mar{\'\i}n}, H{\'e}ctor and {Nore{\~n}a}, Jorge and {Verde}, Licia and {Percival}, Will J. and {Wagner}, Christian and {Manera}, Marc and {Schneider}, Donald P.},
        title = "{The power spectrum and bispectrum of SDSS DR11 BOSS galaxies - I. Bias and gravity}",
      journal = {\mnras},
     keywords = {galaxies: haloes, cosmological parameters, cosmology: theory, large-scale structure of Universe, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = jul,
       volume = {451},
       number = {1},
        pages = {539-580},
          doi = {10.1093/mnras/stv961},
archivePrefix = {arXiv},
       eprint = {1407.5668},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.451..539G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{LinearBiasInsufficient,
       author = {{S{\'a}nchez}, Ariel G. and {Cole}, Shaun},
        title = "{The galaxy power spectrum: precision cosmology from large-scale structure?}",
      journal = {\mnras},
     keywords = {cosmological parameters, large-scale structure of the Universe, Astrophysics},
         year = 2008,
        month = apr,
       volume = {385},
       number = {2},
        pages = {830-840},
          doi = {10.1111/j.1365-2966.2007.12787.x},
archivePrefix = {arXiv},
       eprint = {0708.1517},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008MNRAS.385..830S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Croom2005,
       author = {{Croom}, Scott M. and {Boyle}, B.~J. and {Shanks}, T. and {Smith}, R.~J. and {Miller}, L. and {Outram}, P.~J. and {Loaring}, N.~S. and {Hoyle}, F. and {da {\^A}ngela}, J.},
        title = "{The 2dF QSO Redshift Survey - XIV. Structure and evolution from the two-point correlation function}",
      journal = {\mnras},
     keywords = {galaxies: clusters: general, quasars: general, cosmology: observations, large-scale structure of Universe, Astrophysics},
         year = 2005,
        month = jan,
       volume = {356},
       number = {2},
        pages = {415-438},
          doi = {10.1111/j.1365-2966.2004.08379.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0409314},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005MNRAS.356..415C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fry1996,
       author = {{Fry}, J.~N.},
        title = "{The Evolution of Bias}",
      journal = {\apjl},
     keywords = {COSMOLOGY: LARGE-SCALE STRUCTURE OF UNIVERSE},
         year = 1996,
        month = apr,
       volume = {461},
        pages = {L65},
          doi = {10.1086/310006},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996ApJ...461L..65F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book{Cowan,
  title={Statistical data analysis},
  author={Cowan, Glen},
  year={1998},
  publisher={Oxford university press}
}
